Simplified POMDP Planning with an Alternative Observation Space and Formal Performance Guarantees

Online planning under uncertainty in partially observable domains is an essential capability in robotics and AI. The partially observable Markov decision process (POMDP) is a mathematically principled framework for addressing decision-making problems in this challenging setting. However, finding an optimal solution for POMDPs is computationally expensive and is feasible only for small problems. In this work, we contribute a novel method to simplify POMDPs by switching to an alternative, more compact, observation space and simplified model to speedup planning with formal performance guarantees. We introduce the notion of belief tree topology, which encodes the levels and branches in the tree that use the original and alternative observation space and models. Each belief tree topology comes with its own policy space and planning performance. Our key contribution is to derive bounds between the optimal Q-function of the original POMDP and the simplified tree defined by a given topology with a corresponding simplified policy space. These bounds are then used as an adaptation mechanism between different tree topologies until the optimal action of the original POMDP can be determined. Further, we consider a specific instantiation of our framework, where the alternative observation space and model correspond to a setting where the state is fully observable. We evaluate our approach in simulation, considering exact and approximate POMDP solvers and demonstrating a significant speedup while preserving solution quality. We believe this work opens new exciting avenues for online POMDP planning with formal performance guarantees.

==> logs/00-Proof.tex <==
\subsection*{Proof of Lemma \ref{lemma:bound-q}}
\label{proof-lemma-bound-q}

\begin{theorem}[Lemma 
 \ref{lemma:bound-q}]
 \textbf{Bound Q value.} We can bound the Q function between the closed-loop POMDP belief tree $\topo_C$ and a given adaptive observation topology belief tree $\BelTree^\topo$ with some simplifications.
 \begin{flalign}
     \Delta Q(b_0,\action_0, \policy^{\topo C},\policy^{\topo},\topo_C, \topo)
     \leq 
     \max_{\bpolicy^{\topo}\in \Pi^{\topo}} | Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) | 
     \triangleq
     \delta_Q(b_0,\action_0, \policy^{\topo},\topo) \nonumber
 \end{flalign}
\end{theorem}

\DK{Move proof here.}


\subsection*{Proof of Theorem \ref{theorem:q}}
\label{proof:theorem-q}
\begin{theorem}[Theorem \ref{theorem:q}]
	We can further bound the Q function of the closed-loop POMDP belief tree $\BelTree^{\topo_C}$ by deriving the tightest bound from Lemma \ref{lemma:bound-q}: 
	\begin{flalign}		Q_{\topo_C}^{\policy^{\topo C}}(b_0,\action_0)  & \leq \min_{\policy^{\topo}\in \Pi^{\topo}} [Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) +\delta_Q(b_0,\action_0, \policy^{\topo},\topo) ]\\ & = \min_{\policy^{\topo}\in \Pi^{\topo}} [Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)+\max_{\bpolicy^{\topo}\in \Pi^{\topo}} | Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) |] \label{theorem-q-equ1}
	\\
	& = \max_{\policy^{\topo}\in \Pi^{\topo}}[Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)]\label{theorem-q-equ2}
	% \\		& = Q^{QMDP,*}(b_0, \pi_0)
\end{flalign}
\begin{flalign}		Q_{\topo_C}^{\policy^{\topo C}}(b_0,\action_0)  & \geq \max_{\policy^{\topo}\in \Pi^{\topo}} [Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) -\delta_Q(b_0,\action_0, \policy^{\topo},\topo) ]\\ & = \max_{\policy^{\topo}\in \Pi^{\topo}} [Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)-\max_{\bpolicy^{\topo}\in\Pi^{\topo}} | Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) |] \label{theorem-q-equ3} \\
	& = \min_{\policy^{\topo}\in \Pi^{\topo}}[Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)]
\end{flalign}
\end{theorem}
\begin{proof}
Here we show how to get (\ref{theorem-q-equ2}) from (\ref{theorem-q-equ1}). We consider both possible cases to prove this.
	
Firstly, if assuming 
 \begin{equation}
     |Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) - \min_{\bpolicy^{\topo}\in \Pi^{\topo}}Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0)|\leq |Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) - \max_{\bpolicy^{\topo}\in \Pi^{\topo}}Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0)   | 
 \end{equation} 
	, so we have: \begin{equation}
	    \max_{\bpolicy^{\topo}\in \Pi^{\topo}} | Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) |=|Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) - \max_{\bpolicy^{\topo}\in \Pi^{\topo}}Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0)|
	\end{equation}
	
Then we can get:
	\begin{flalign}
		\min_{\policy^{\topo}\in\Pi^{\topo}} &[Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)+\max_{\bpolicy^{\topo}\in \Pi^{\topo}} | Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) |]  \nonumber \\ &=
		\min_{\policy^{\topo}\in\Pi^{\topo}} [Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)+\max_{\bpolicy^{\topo}\in \Pi^{\topo}}  Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) ] 
		\\ & =  \max_{\bpolicy^{\topo}\in \Pi^{\topo}}  Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0)
	\end{flalign}
	
Secondly, if assuming 
 \begin{equation}
     |Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) - \min_{\bpolicy^{\topo}\in\Pi^{\topo}}Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0)|\geq |Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) - \max_{\bpolicy^{\topo}\in \Pi^{\topo}}Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0)   |
 \end{equation}
 It means that $2Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)  \geq \min_{\bpolicy^{\topo}\in\Pi^{\topo}}Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0)+ \max_{\bpolicy^{\topo}\in \Pi^{\topo}}Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) $.
Then we will have:
\begin{flalign}
\min_{\policy^{\topo}\in\Pi^{\topo}} &[Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)+\max_{\bpolicy^{\topo}\in \Pi^{\topo}} | Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) |]\nonumber \\
&=    	\min_{\policy^{\topo}\in\Pi^{\topo}} [Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)-\min_{\bpolicy^{\topo}\in\Pi^{\topo}}  Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) + Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) ] \\
& =  \min_{\policy^{\topo}\in\Pi^{\topo}} [2Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)]-\min_{\bpolicy^{\topo}\in\Pi^{\topo}}  Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) \\
& = \max_{\bpolicy^{\topo}\in \Pi^{\topo}}Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) 
\end{flalign}
\end{proof}

\subsection*{Proof of Lemma \ref{lemma:bound-optimal}}
\label{proof:lemma-optimal}
\begin{theorem}[Lemma \ref{lemma:bound-optimal}]
	\textbf{Bound the optimal Q function.} 
	For a certain topology belief tree $\topo$, if the belief node $b^{\topo-}_{i+1}$,
	The lower bound of the optimal policy within the closed-loop POMDP belief tree $\topo_C$ can be calculated in the iterative way below. We define the lower bound for the optimal Q-function for a pure closed-loop POMDP belief tree $Q_{\topo_C}^{*}(b_0,\action_0)$ as $lq(b_0, \action_0, \topo)$:
	\begin{flalign}
		Q_{\topo_C}^{*}(b_0,\action_0) \geq lq(b_0, u_0, \topo)
	\end{flalign}
	where, the lower bound function is defined iteratively as:
	\begin{flalign}
		lq(b_t, \action_t, \topo) := &\indicator_{\simpfunc(\shis^{\topo}(b^-_{t+1}))=1}[r(b_{t},\action_t) +\exptsimp{z_{t+1}|\shis^{\topo}(b_{t}),\action_t}{\topo} \max_{\policy_{t+1}}lq(b_{t+1},\policy_{t+1},\topo)]\nonumber \\
		+& \indicator_{\simpfunc(\shis^{\topo}(b^-_{t+1}))=0}[r(b_{t},\action_t) +\exptsimp{z_{t+1}|\shis^{\topo}(b_{t}),\action_t}{\topo} \min_{\policy_{t}}lq(b_{t+1},\policy_{t+1},\topo)]
		\label{equ:optimal-lower-bound}
	\end{flalign} 
\end{theorem}
\begin{proof}
Let's consider the end of the planning horizon $L$.

If $\simpfunc^{\topo}(\shis(b^-_{L-1}))=1$, we have:
\begin{flalign}
\int_{z_{L-1}}p(z_{L-1}|x_{L-1})\max_{\policy^{\topo}_{L-1}\in\Pi^{\topo}}\int_{x_L}p(x_L|x_{L-1},\policy^{\topo}_{L-1}) = \int_{z_{L-1}}p(z_{L-1}|x_{L-1})\int_{x_L}p(x_L|x_{L-1},\policy^{\topo_C*}_{L-1}) 
    \label{equ:opti-1}
\end{flalign}
If $\simpfunc^{\topo}(\shis(b^-_{L-1}))=0$, we have:
\begin{flalign}
\min_{\policy^{\topo}_{L-1}\in\Pi^{\topo}}\int_{x_L}p(x_L|x_{L-1},\policy^{\topo}_{L-1}) \leq \int_{z_{L-1}}p(z_{L-1}|x_{L-1})\int_{x_L}p(x_L|x_{L-1},\policy^{\topo_C*}_{L-1}) 
\label{equ:opti-2}
\end{flalign}
We denote the left-hand side in Equation (\ref{equ:opti-1}) and (\ref{equ:opti-2}) as $LHS1(x_{L-1}, \topo)$ and the right-hand side as $RHS1(x_{L-1}, \topo_C)$. In general, we can say $LHS1(x_{L-1}, \topo) \leq RHS1(x_{L-1}, \topo_C)$. 

Then, we take one more step earlier. Also if
 %$b^-_{L-2}\in\obsNodeNot_{L-2}^{\topo}$
$\simpfunc^{\topo}(\shis(b^-_{L-2}))=1$
 , we have:
\begin{flalign}
\nonumber\int_{z_{L-1}}&p(z_{L-1}|x_{L-1})
\max_{\policy_{L-2}^{\topo}\in\Pi^{\topo}}\int_{x_{L-1}}p(x_{L-1}|x_{L-2},\policy_{L-2}^{\topo})[r(x_{L-1})+LHS1(x_{L-1}, \topo)] \\
& \leq \int_{z_{L-2}}p(z_{L-2}|h_{L-2})\int_{x_{L-2}}p(x_{L-2}|x_{L-2},\policy_{L-2}^{\topo_C*})[r(x_{L-1})+RHS1(x_{L-1}, \topo)]
\label{equ:opti-3}
\end{flalign}
And if $\simpfunc^{\topo}(\shis(b^-_{L-2}))=0$, we have:
\begin{flalign}
\min_{\policy_{L-2}^{\topo}\in\Pi^{\topo}}&\int_{x_{L-1}}p(x_{L-1}|x_{L-2},\policy_{L-2}^{\topo})[r(x_{L-1})+LHS1(x_{L-1}, \topo)]\nonumber \\
& \leq \int_{z_{L-2}}p(z_{L-2}|h_{L-2})\int_{x_{L-2}}p(x_{L-2}|x_{L-2},\policy_{L-2}^{\topo_C*})[r(x_{L-1})+RHS1(x_{L-1}, \topo)]
\label{equ:opti-4}
\end{flalign}
We also denote the left-hand side of the inequality in Equation (\ref{equ:opti-3}) and (\ref{equ:opti-4}) as $LHS2(x_{L-2}, \topo)$ and the right-hand side as $RHS2(x_{L-2}, \topo_C)$. In general, we can say $LHS2(x_{L-2}, \topo) \leq RHS2(x_{L-2}, \topo_C)$. 

The left-hand side is the iterative way to calculate $lq(b_t,\policy_t,\topo)$. If we keep iterate the above process from the end to the beginning of the planning horizon, we will get the inequality at the top of the belief tree:  $ lq(b_0, \action_0, \topo) \leq Q_{\topo_C}^{\policy^{\topo_C*}}(b_0,\action_0) $.
     	
% Blow is some process that is not used for proof.
%       \begin{flalign}
% Q_{\topo_C}^{\policy^{\topo_C*}_{i+1:L}}(b_i,\policy_i)  & = \emathbb{x_{i+1}|b_i,\policy_i}r(x_{i+1}) +  \emathbb{z_{i+1}|b_i,\policy_i,\topo_C}\max_{\policy_{i+1}}[ Q_{\topo_C}^{\policy^{\topo_C*}_{i+2:L}}(b_{i+1},\policy_{i+1})] \\& \geq \emathbb{x_{i+1}|b_i,\policy_i}r(x_{i+1})+\emathbb{z_{i+1}|b_i,\policy_i,\topo_C}\max_{\policy_{i+1}}\{ \min_{\policy^{\topo}_{i+2:L}}[Q_{\topo}^{\policy^{\topo}_{i+2:L}}(b_{i+1},\policy_{i+1})]\} 
% % & = r(b_i)+\emathbb{z_{i+1}|b_i,\policy_i}{\topo}\max_{\policy_{i+1}}\{ \min_{\policy^{\topo}_{i+2:L}}[Q_{\topo}^{\policy^{\topo}_{i+2:L}}(b_{i+1},\policy_{i+1})]\}
% 	\end{flalign}	
% 	\begin{flalign}
% \emathbb{z_1:i,\topo_C}&\max_{\policy^{\topo_C}_i}Q_{\topo_C}^{\policy^{\topo_C*}_{i+1:L}}(b_i,\policy_i)   = \emathbb{z_1:i,\topo_C}\max_{\policy^{\topo_C}_i}\Big[\emathbb{x_{i+1}|b_i,\policy_i}r(x_{i+1}) +  \emathbb{z_{i+1}|b_i,\policy_i,\topo_C}\max_{\policy_{i+1}}[ Q_{\topo_C}^{\policy^{\topo_C*}_{i+2:L}}(b_{i+1},\policy_{i+1})] \Big]\\& \geq  \emathbb{z_1:i,\topo_C}\max_{\policy^{\topo_C}_i}\Big[\emathbb{x_{i+1}|b_i,\policy_i}r(x_{i+1})+\emathbb{z_{i+1}|b_i,\policy_i,\topo_C}\max_{\policy_{i+1}}\{ \min_{\policy^{\topo}_{i+2:L}}[Q_{\topo}^{\policy^{\topo}_{i+2:L}}(b_{i+1},\policy_{i+1})]\}\Big] \\
% & = \emathbb{z_1:i,\topo_C}\max_{\policy^{\topo_C}_i}\Big[\emathbb{x_{i+1}|b_i,\policy_i}r(x_{i+1})+\emathbb{z_{i+1}|b_i,\policy_i}{\topo}\max_{\policy_{i+1}}\{ \min_{\policy^{\topo}_{i+2:L}}[Q_{\topo}^{\policy^{\topo}_{i+2:L}}(b_{i+1},\policy_{i+1})]\} \Big] \\
% & = \emathbb{z_1:i|b_0,\policy^{\topo_C*}_{1:i-1}} {\topo_C}\max_{\policy^{\topo_C}_i}\emathbb{x_{i+1}|b_i,\policy_i}r(x_{i+1}) + \emathbb{z_1:i|b_0,\policy^{\topo_C*}_{1:i-1},\topo_C} \max_{\policy^{\topo_C}_i}\max_{\policy_{i+1}}\{ \min_{\policy^{\topo}_{i+2:L}}[Q_{\topo}^{\policy^{\topo}_{i+2:L}}(b_{i+1},\policy_{i+1})]\} \\
% & \geq \min_{\policy_{1:i}^{\topo}} \emathbb{z_1:i|b_0,\policy_{1:i+1}^{\topo}}{\topo}r(b_{i+1})
% 	\end{flalign}	

\end{proof}


\subsection*{Proof of Theorem \ref{theorem:upper-bound-estimation}}
\label{proof: upper-bound-estimation}
\begin{theorem}
	[Theorem \ref{theorem:upper-bound-estimation}] \textbf{Bounded Estimation Error.} For all the depth $d=0,...,L-1$ and $a$, the following concentration bound holds with probability at least $1-|A|(|A|C)^L\exp(\frac{-C\lambda^2}{2V_{\max}^2})$ :
	\begin{flalign}
		\Delta \hat{uq}(b_0,a_0, \topo) \leq \frac{L(L-1)}{2}\lambda \nonumber
	\end{flalign}
\end{theorem}
\begin{proof}
    We will follow a similar way to prove it as \cite{Kearns02jml, Lim23jair}.

    Firstly, we consider a general situation at a depth of $d$ and try to bound the error of estimating the optimal Q function given a belief $b_d$ and an action $a_d$:
    \begin{flalign}
       \delta^{\topo}_{\Hat{uq}}(d) &\triangleq |{Q}_{\topo}^{\policy^{\topo*}}(b_d,\action_d)-\hat{Q}_{\topo}^{\policy^{\topo*}}(b_d,\action_d) | \\& = \Big|r(b_d,\action_d) +  \emathbb{b_{d+1}|b_d,\action_d}[V^{\topo*}(b_{d+1})] - r(b_d, \action_d) - \frac{1}{C}\sum_{i=1}^{C}\hat{V}^{\topo*}(b_{d+1}'^{[I_i]})\Big|\\
        &=\Big|\emathbb{z_{d+1}|b_d,\action_d,\topo}[V^{\topo*}(b_{d+1})] - \frac{1}{C}\sum_{i=1}^{C}\hat{V}^{\topo*}(\Bar{b}_{d+1}^{\topo, [I_i]})\Big| \\
        & \leq \Big| \emathbb{z_{d+1}|b_d,\action_d,\topo}[V^{\topo*}(b_{d+1})] -  \frac{1}{C}\sum_{i=1}^{C}V^{\topo*}(\Bar{b}_{d+1}^{\topo, [I_i]}) \Big|+\Big| \frac{1}{C}\sum_{i=1}^{C}V^{\topo*}(\Bar{b}_{d+1}^{\topo, [I_i]}) -  \frac{1}{C}\sum_{i=1}^{C}\hat{V}^{\topo*}(\Bar{b}_{d+1}^{\topo, [I_i]}) \Big| \label{equ:esti-1}
    \end{flalign}

Here, the propagated next step belief state samples for a given belief tree topology $\topo$ is denoted as $\Bar{b}_{d+1}^{\topo, [I_i]}$. It is updated by the motion and observation models for the given topology $\topo$:
\begin{equation}
     \Bar{b}_{d+1}^{\topo, [I_i]} \sim
     \psi^{\topo}(\Bar{b}_{d+1}^{\topo} | b_d, \action_d) =
     \indicator_{\simpfunc(h^-_{d+1})=1}\alpha\cdot \prob{z_{d+1}|x_{d+1}}\prob{x_{d+1}|b_d, a_d} + \indicator_{\simpfunc(h^-_{d+1})=0}\prob{x_{d+1}|b_d, a_d}
\end{equation}
Here, $\alpha$ is a Bayes normalization factor.
For the first term in Equation (\ref{equ:esti-1}), we can directly use the Hoeffding's inequality:
\begin{flalign}
\prob{\Big|\emathbb{z_{d+1}|b_d,\action_d,\topo}[V^{\topo*}(b_{d+1})] -  \frac{1}{C}\sum_{i=1}^{C}V^{\topo*}(b_{d+1}'^{[I_i]})\Big| \leq \lambda } \geq 1- 2 \exp(\frac{-C\lambda^2}{2V_{\max}^2})
\end{flalign}

For the second term in Equation (\ref{equ:esti-1}), we analyze it in an iterative way:
\begin{flalign}
    \Big| \frac{1}{C}\sum_{i=1}^{C}V^{\topo*}(\Bar{b}_{d+1}^{\topo, [I_i]}) -  \frac{1}{C}\sum_{i=1}^{C}\hat{V}^{\topo*}(\Bar{b}_{d+1}^{\topo, [I_i]}) \Big| &= \frac{1}{C}\Big| \sum_{i=1}^{C}Q_{\topo}^{\policy^{\topo*}}(\Bar{b}_{d+1}^{\topo, [I_i]}, \action^*_{d+1})- \sum_{i=1}^{C}\hat{Q}_{\topo}^{\policy^{\topo*}}(\Bar{b}_{d+1}^{\topo, [I_i]}, \action^*_{d+1}) \Big| \\
    &\leq \delta^{\topo}_{\Hat{uq}}(d+1)
\end{flalign}

So, the below iterative bound is satisfied with a probability of at least $1-|A|(|A|C)^L\exp(\frac{-C\lambda^2}{2V_{\max}^2})$:
\begin{flalign}
    \delta^{\topo}_{\Hat{uq}}(d) \leq \lambda +  \delta^{\topo}_{\Hat{uq}}(d+1)
    \label{equ:esti-2}
\end{flalign}
The estimation error at the end is:
\begin{equation}
    \delta^{\topo}_{\Hat{uq}}(L-1) = 0 
\end{equation}

Then, we can find out the estimation bound at the top of the given belief tree by calculating it from the bottom to the top by Equation (\ref{equ:esti-2}).
\end{proof}

\subsection*{Proof of Theorem \ref{theorem:lower-bound-estimation}}
\label{proof: lower-bound-estimation}
\begin{theorem}
	[Theorem \ref{theorem:lower-bound-estimation}] \textbf{Estimation bound of the lower bound.} For all the depth $d= 0,..., L-1$ and $\action$, the following concentration bound holds with probability at least $1-|A|(|A|C)^L\exp(\frac{-C\lambda^2}{2V_{\max}^2})$:
	\begin{equation}
		\Delta \hat{lq}(b_0,a_0, \topo) \leq \frac{L(L-1)}{2}\lambda \nonumber
	\end{equation}
\end{theorem}
\begin{proof}
	Firstly, we consider a general situation at a depth of $d$ and try to bound the error of estimating the lower bound function given a belief $b_d$ and an action $a_d$:
	\begin{flalign}
		\delta^{\topo}_{lq}(t) \triangleq|&{lq}(b_t,a_t, \topo) - \hat{lq}(b_t,a_t, \topo)| \\=\Big|&\indicator_{\simpfunc(\shis(b^-_{t+1}))=1}\big[\emathbb{z_{t+1}|\shis(b_{t}),\action_t,\topo}\max_{\policy_{t+1}}lq(b_{t+1},\policy_{t+1},\topo)- \frac{1}{C}\sum_{i=1}^{C}\max_{\policy_{t+1}}\hat{lq}(\Bar{b}^{I_i}_{t+1},\policy_{t+1},\topo)\big]\nonumber \\
		+ &\indicator_{\simpfunc(\shis(b^-_{t+1}))=0}\big[\emathbb{z_{t+1}|\shis(b_{t}),\action_t,\topo} \min_{\policy_{t+1}}lq(b_{t+1},\policy_{t+1},\topo)-\frac{1}{C}\sum_{i=1}^{C} \min_{\policy_{t+1}}\hat{lq}(\Bar{b}^{I_i}_{t+1},\policy_{t+1},\topo)\big]\Big|\\
		\leq \Big|&\indicator_{\simpfunc(\shis(b^-_{t+1}))=1}\{\big| \emathbb{z_{t+1}|\shis(b_{t}),\action_t,\topo}\max_{\policy_{t+1}}lq(b_{t+1},\policy_{t+1},\topo) - \frac{1}{C}\sum_{i=1}^{C}\max_{\policy_{t+1}}lq(\Bar{b}^{I_i}_{t+1},\policy_{t+1},\topo) \big|\nonumber
		\\ &+ \ \big|\frac{1}{C}\sum_{i=1}^{C}\max_{\policy_{t+1}}lq(\Bar{b}^{I_i}_{t+1},\policy_{t+1},\topo) - \frac{1}{C}\sum_{i=1}^{C}\max_{\policy_{t+1}}\hat{lq}(\Bar{b}^{I_i}_{t+1},\policy_{t+1},\topo)\big| \} \nonumber
		\\
		+ &\indicator_{\simpfunc(\shis(b^-_{t+1}))=0}   \{\big| \emathbb{z_{t+1}|\shis(b_{t}),\action_t,\topo}\min_{\policy_{t+1}}lq(b_{t+1},\policy_{t+1},\topo) - \frac{1}{C}\sum_{i=1}^{C}\min_{\policy_{t+1}}lq(\Bar{b}^{I_i}_{t+1},\policy_{t+1},\topo) \big| \nonumber
		\\ &+ \big|\frac{1}{C}\sum_{i=1}^{C}\min_{\policy_{t+1}}lq(\Bar{b}^{I_i}_{t+1},\policy_{t+1},\topo) - \frac{1}{C}\sum_{i=1}^{C}\min_{\policy_{t+1}}\hat{lq}(\Bar{b}^{I_i}_{t+1},\policy_{t+1},\topo) \big|\} \Big| \label{equ:lq-lambda-pre}
	\end{flalign}
	Here, we can use a technique similar to the previous proof. We can directly use the Hoeffding inequality to bound the first term in each indicator as:
	\begin{equation}
		\prob{\Big|\emathbb{z_{t+1}|\shis(b_{t}),\action_t,\topo}\max_{\policy_{t+1}}lq(b_{t+1},\policy_{t+1},\topo) - \frac{1}{C}\sum_{i=1}^{C}\max_{\policy_{t+1}}lq(\Bar{b}^{I_i}_{t+1},\policy_{t+1},\topo)\Big| \leq \lambda } \geq 1- 2 \exp(\frac{-C\lambda^2}{2V_{\max}^2})
	\end{equation}
	\begin{equation}
		\prob{\Big|
			\emathbb{z_{t+1}|\shis(b_{t}),\action_t,\topo}\min_{\policy_{t+1}}lq(b_{t+1},\policy_{t+1},\topo) - \frac{1}{C}\sum_{i=1}^{C}\min_{\policy_{t+1}}lq(\Bar{b}^{I_i}_{t+1},\policy_{t+1},\topo)
			\Big| \leq \lambda } \geq 1- 2 \exp(\frac{-C\lambda^2}{2V_{\max}^2})
	\end{equation}
 The second term is also iteratively bounded by  $\delta^{\topo}_{lq}(t+1)$.
	So, combining the two probabilistic bounds together, we can get the iterative bound for the estimator satisfied with a probability of at least $1-|A|(|A|C)^L\exp(\frac{-C\lambda^2}{2V_{\max}^2})$:
	\begin{flalign}
		\delta^{\topo}_{lq}(t)\leq (\ref{equ:lq-lambda-pre})\leq &\indicator_{\simpfunc(\shis(b^-_{t+1}))=1} \big[\lambda + \delta^{\topo}_{lq}(t+1)\big] + \indicator_{\simpfunc(\shis(b^-_{t+1}))=0} \big[\lambda + \delta^{\topo}_{lq}(t+1)\big]\label{equ:lq-lambda} \\
		= &  \lambda + \delta^{\topo}_{lq}(t+1)
	\end{flalign}
	The estimate error at the end of the planning horizon is:
	\begin{equation}
		\delta^{\topo}_{lq}(L-1) = 0
	\end{equation}
	Now, we can find out the estimation bound at the top of the given belief tree by calculating it from the bottom to the top, from $L-1$ to $0$.
\end{proof}

==> logs/01-Intro.tex <==

The real-world robotics applications face the challenges of planning under uncertainty due to imperfect state estimation results. 
It has long been regarded as a difficult but fundamental problem, especially for the navigation of autonomous systems, e.g., active SLAM \cite{Placed23tro}.

The Partially Observable Markov Decision Process (POMDP)~\cite{Kaelbling98ai} is a promising mathematics pipeline for decision-making under uncertainty, assuming that the underlying system dynamics are governed by a Markov Decision Process (MDP) model and that the states are not fully observable.
It models the robot as an \textit{agent} with imperfect state estimation information to derive a solution, named \textit{policy}, deciding the optimal actions based on the agent's history of actions and observations. 
Instead, one should maintain a \textit{belief}, which is a probability distribution function over the underlying states.
By considering all kinds of uncertainty and planning in the belief space, POMDP has shown proven advantages in general decision-making problems under uncertainty and many robotics tasks \cite{Lauri22tro}.
It can support numerous tasks in robotics, such as autonomous navigation, where the states and observations of the agent are uncertain due to the noise of sensors and limited perception.

\DK{Also need to introduce the idea of switching / alternative observation space and model.}
However, solving a full POMDP is intractable due to its complexity. The dimension grows exponentially with the number of the state, which is called \textit{the curse of dimensionality}. The size of the belief tree will also grow exponentially with the planning horizon, which is called \textit{the curse of history}.
Consequently, simplified \cite{Sztyglic22iros} or approximate methods have become indispensable for real-world robotic applications of POMDPs, usually providing near-optimal policies \cite{Kara22jmlr}.
Efforts to simplify POMDPs have focused on various aspects, including:
finite memory of history \cite{Kara22jmlr} to ease the curse of time, finite information state space\cite{Subramanian19cdc}, and the simplified belief space\cite{Lee07nips}. 

\DK{Address more on the performance guarantee.}
Moreover, it is imperative to provide a rigorous theoretical demonstration that the simplified or approximated models can effectively represent the original POMDP and establish a performance guarantee.
The performance guarantee of a POMDP is typically defined as... 
However, only some of the simplification methods offer theoretical performance guarantees, many lack such assurances, highlighting the need for careful evaluation in practical settings. 
Some of the methods can provide a performance guarantee, but many of them cannot. 
The performance guarantee of POMDP is defined in ...


In many robotics applications, such as those involving image input or visual SLAM \cite{Giuliari21iros}, observation models can be complex. 
Simplification strategies often focus on using a simpler model \cite{Lev24aaai} or identifying a relevant subset of the full observation space \cite{Barenboim24nips}."
\DK{Add more citations here.}


Barenboim \cite{Barenboim24nips} provides a general deterministic bound for simplifications of the observation model by sparsifying the observation space. 
Lev-Yehudi \cite{Lev24aaai} used a simplified observation model for planning and provided a performance guarantee. 

Contrast to the existing method, we propose to switch the observation model and space together to the different but simpler ones, creating the \textit{latent observation}. It means the planner does not have to reason the whole observation space in some steps.  
This adaptive simplification structure will help reduce the dimensionality of the policy space. 
We provide a performance guarantee along with our simplification scheme, showing our method can achieve the same optimal policy with simplified policy space. With our adaptive simplification scheme, we also demonstrate the connection with QMDP and open-loop planning, showing the underlying pipeline of simplification of observation model.


\subsection*{Contribution statement}

1. We propose an adaptive simplification method for the observation model and the observation space. Based on this, a novel Adaptive Observation Topology Belief Tree is presented.
We are the first to propose a switching strategy to simplify the observation model.

2. We derive a bound between our proposed Adaptive Observation Topology Belief Tree and the common full POMDP belief tree. 

3. Based on this bound, we present a simplification method for POMDP regarding the simplified observation model and space and provide a performance guarantee.

4. We explore different levels of simplification to enable online simplification for POMDP.

5. We run multiple experiments to support our analysis.





==> logs/02-Background.tex <==
\subsection{Related Work}

\subsubsection{Simplification and approximation of POMDP}

Here, we survey the simplification and approximation of POMDPs. Many perspectives of POMDPs can be simplified, including sampling-based, memory history, and infomration states.

Hoerger \cite{Hoerger23ijrr} proposed a multi-level approximation of POMDP.

Kara \cite{Kara22jmlr} tries to approximate POMDP by reducing its history memory, and proves the near optimality of finite memory feedback policies.
They prove the near optimality from the perspective of filter stability.
% Their proof is mainly based on the Bounded Lipschitz metric rather than Total Variation. 
% The bound of expectation difference is bounded by the BL metric of differences in the beginning belief of the N-step window.
% Their proof is general and rigorous, which is inspiring to the proof of adaptive open-loop planning. For example, we can treat the bounding problem as the filter stabilization problem, bounding the whole reward with the differences of belief.
Similarly, in the context of the partially observable control system, Subramanian\cite{Subramanian19cdc} tried to simplify the information states.
% However, their method is a kind of \textit{ uniform quantization}(See \cite{Kara22jmlr}, pg.11-12 ), which means that for any belief $b \in \mathcal{B}$, there exists a simplified belief $\hat{b} \in \mathcal{\hat{B}}$ with $|| b - \hat{b} || \leq \epsilon$ for a fixed $\epsilon$.
% Note that the metric used here is determined by the state space $\mathcal{X}$: total variation (L1 distance) for finite $\mathcal{X}$ and bounded Lipschtz metric for a general $\mathcal{X}$. (See \cite{Kara22jmlr}, pg.12) 
% Also, Remark 8 in \cite{Kara22jmlr} discusses the bounds.
% Another Kara paper\cite{Kara22math} proposes a TV-distance-based bounding term (see Equation 16 in \cite{Kara22math}). 
% The TV bound is looser than the BL (bounded Lipschtz) bound and always upper bounds the BL bound, but cheaper to calculate. 




\subsubsection{QMDP and Open-Loop Planning}


The topic of open-loop planning was first brought out in the field of reinforcement learning as 
\textit{Option} \cite{Sutton99ai}.
In the context of POMDP, Flaspohler et al. \cite{Flaspohler20nips} used the concept of VoI (Value of Information) to evaluate the observations in closed-loop steps compared to open-loop steps.
However, the computational cost of calculating the VoI is significant, and thus the potential for resource savings is limited.

From the perspective of bounding the robot motion control, Majumdar\cite{Majumdar23ijrr} tries to bound the motion model, which can be viewed as a bound for open-loop planning and POMDP.
They use f-informativity to analyze the bound of reward. 
% Based on the assumption of bounded rewards (i.e., the normalized reward $r_n = \frac{r}{R_{max}} \in [0,1]$), they use some theorems for f-divergence of Bernoulli distributions.  
% I think their results come from the full exploitation of the assumption of bounded rewards.
% It is very tricky to fully exploit the bounded reward such that some theorems for Berllouni distribution can be used to construct a Fano's inequality. (Any lower bound of f-informativity can lead to a Fano's style inequality)

Hauser\cite{Hauser10wafr, Hauser11icml} used the QMDP approximation as the open-loop information searching process.

\textit{Macro action} and \textit{durative action} are two relative concepts, where the action sequence comprising different actions and the same action are pre-decided.
Durative action in POMDP is another interpretation of  macro-action.\cite{Khonji23aaai, Mann15jair}
Besides, some practical work focus on learning based method to generate the macro-action sequences like \cite{Liang23iros, Lee21rss}. While, these learning based methods still lack the analysis of performance guarantees.


\subsubsection{Simplified POMDP with performance guarantees}

Many works have been proposed to preserve the performance guarantees after simplification\cite{Zhitnikov23arxiv,Lim23jair}.

\subsection{POMDP Model}

The basic model of POMDP is defined as a tuple:
$<\CX, \CA, \Zspace, \mathbb{P}_{T}, \mathbb{P}_{Z}, r>$, where $\CX$ is the state space, $\CA$ is the action space, $\Zspace$ is the observation space.
%and $\action$ is the action sequence, with open-loop actions or closed-loop policies, decided by the sequence parameter $\seqParam$. 
 The transition model (or motion model) is defined as $\mathbb{P}_{T}(x_{k+1}|x_k, a_k)$, which describes the probabilistic transition of the state from $x_k\in\CX$ to $x_{k+1}\in\CX$ under a certain action $a_k \in \CA$. The observation model is defined as $\probz{z_k|x_k}$, which describes the probability of observation $z_k\in\Zspace$ given a certain state $x_k\in\CX$.
 The reward function is considered to be state dependent, $r: \mathcal{X},\mathcal{A} \mapsto \mathbb{R}$, and holds the bounded reward assumption: $r \in [-R_{\max}, R_{\max}]$. 

Given that the true state is uncertain, a belief is maintained to represent the distribution of the current state with regard to history.
The belief at the time of $k$ is defined as $b_k \triangleq \prob{x_{k}| h_{k}} $, where $h_{k}$ is the history until the time $k$ as $h_{k} \triangleq \{z_{1:k},a_{0:k-1}\}$. A propagated history without the latest observation $h_k^{-}$ is defined as: $h_k^{-} = \{z_{1:k-1},a_{0:k-1}\}$, and the corresponding propagated belief is $b^-_k \triangleq \prob{x_k|h^-_k}$.

A policy function is defined as $\pi:\mathcal{H}\to\CA$, which decides actions based on the history of beliefs. The value function for a certain policy $\pi$ over the planning horizon $L$ is defined as the summation of all expected rewards:
\begin{equation}
    V^\pi(b_k)= r(b_k, \pi_k(b_k)) + \sum_{i=k+1}^{   L}\emathbb{z_{k+1:i}}\big[ r(b_i,\pi_i(b_i))\big]
\end{equation}
The goal of a POMDP is to find the optimal policy $\pi^*$ that maximizes the value function. The optimal policy can be calculated by the Bellman optimality as:
\begin{equation}
    V^{\pi*}(b_k) = \max_{a_k} \Big[ r(b_k, a_k) + \emathbb{z_{k+1}} V^{\pi*}(b_{k+1})\Big]
\end{equation}

% \subsection{Simplification of Observation Model and Space}
% For original observation model:
% \begin{equation}
%     p(z|x): z\in\Zspace 
% \end{equation}
% We can come up with a simplification of the model itself. But also simplifying the model and the observation space at the same time:
% \begin{equation}
%     q(o|x): o \in \CX \text{ or } \Tilde{\mathcal{Z}}
%     \end{equation}

%     For a given history $h_i^-$, we find the optimal policy based on the simplified observation model:
%     \begin{flalign}
%         \emathbb{x_i|h^-_i} \emathbb{o_i|x_i} \emathbb{x_{i+1}|x_i, \pi_i(h_i^-, o_i)} r(x_{i+1}) &\leq \emathbb{x_i|h^-_i} \emathbb{o_i|x_i} \emathbb{x_{i+1}|x_i, \pi^*_i(h_i^-, o_i)} r(x_{i+1}) \\
%         & = \emathbb{x_i|h^-_i} \emathbb{o_i|x_i} \max_{a_i}\emathbb{x_{i+1}|x_i, a_i} r(x_{i+1})
%     \end{flalign}

% For the regular unsimplified policy, we have:
%     \begin{flalign}
%         \emathbb{x_i|h^-_i} \emathbb{z_i|x_i} \emathbb{x_{i+1}|x_i, \pi_i(h_i^-, z_i)} r(x_{i+1}) &\leq \emathbb{x_i|h^-_i} \emathbb{z_i|x_i} \emathbb{x_{i+1}|x_i, \pi^*_i(h_i^-, z_i)} r(x_{i+1}) \\
%         & = \emathbb{x_i|h^-_i} \emathbb{z_i|x_i} \max_{a_i}\emathbb{x_{i+1}|x_i, a_i} r(x_{i+1})
%     \end{flalign}




% \begin{flalign}
% 	\action_{0:L-1}^{*} =\argmax_{\action_{0:L-1}} \emathbb{z_{1:L}}\big[\sum_{i=1}^{L-1} r(b_i, \action_i)\big|\seqParam_{1:L-1} \big]
% \end{flalign} 






%We define the set of observations added into the belief tree as:
%\begin{equation}
%	\hat{Z} = \{ z_t| \seqParam_t(b_t)=1 \}
%\end{equation}
 %the belief in the hybrid belief tree as,
%\begin{flalign}
 %       b_i & = \prob{x_i|b_0, \action_{0:i-1}, z_{0:i}\otimes\seqParam_{0:i} } 
%\end{flalign}



==> logs/03-Method.tex <==
\subsection{Definition of Adaptive Observation Topology Belief Tree}
In this paper, we formulate an Adaptive Observation Topology Belief Tree (AOT-Tree), which is based on an adaptive topology of the belief tree where parts of the belief nodes have a simplified observation model and observation space. 
Figure \ref{fig:belief-tree} demonstrates an example of the proposed Adaptive Observation Topology Belief Tree. 


%\begin{figure}[tb]
%	\includegraphics[width=6cm]{Figures/tree.png}
%	\caption{An Adaptive Observation Topology Belief Tree}
%	\centering
%	\label{fig:belief-tree}
%\end{figure}

\begin{figure}[tb]
	\centering
	\begin{subfigure}[b]{0.45\textwidth} 
		\includegraphics[width=\textwidth]{Figures/p1-qmdp.png} 
		\caption{An Adaptive Observation Topology Belief Tree Simplified for Full Observability}
	\end{subfigure}
	\hfill 
	\begin{subfigure}[b]{0.45\textwidth} 
		\includegraphics[width=\textwidth]{Figures/tree.png} 
		\caption{An Adaptive Observation Topology Belief Tree Simplified for Open-Loop Planning}
	\end{subfigure}
	\caption{Two Examples for the Adaptive Observation Topology Belief Tree. In (a), the left branch has the full observability assumption, where the observation can reveal the true underlying state. While in (b), the left branch uses open-loop actions, where no observation nor state will be considered. } 
		\label{fig:belief-tree}
\end{figure}

We denote the posterior belief node within the Adaptive Observation Topology Belief Tree as $\tb$ and the propagated belief nodes as $\tbm$.
Firstly, we begin with a general definition for the posterior belief $\tb_t$ at time $t$ with regard to its history $\shis_t(\tb_t)$: $\tb_t= \prob{x_t| \shis_t(\tb_t)}$.
We denote the propagated belief immediately after executing the previous action $a_{t-1}$ as $\tbm_t$. 
For simplicity, we denote the history $\shis_t(\tb_t)$ as $h_t$, and the propagated history $\shis_t(\tbm_t)$ as $h_t^-$. 
Here we define the history at a particular belief node as the initial belief $b_0$ and a sequence of all the actions and observations that have been made to reach this belief node from $b_0$.

We denote the simplified observation as $o \in \Ospace$, contrasting to the original observation $z\in\Zspace$. The simplified Observation Space $\Ospace$ is a different general space and not necessary to be a subset of the original observation space $\Zspace$.
The simplified observation model denoted as $\prob{o|x}$ is also completely different from the original observation model $\probz{z|x}$. It depends on how we define the simplified observation space $\Ospace$. 

We define the topology $\topo$ and the corresponding theoretical belief tree $\BelTree^{\topo}$ as follows. The topology is defined in terms of binary variables $\simpfunc^{\topo}(h^{\topo-}_t)\in \{0,1\}$ that indicate each belief node $b^{\topo-}_t$ with the corresponding propagated history $h^{\tau-}_t$ in the belief tree $\BelTree^{\tau}$  whether or not has a simplified observation model and observation space.
Specifically, if $\simpfunc^{\topo}(h^{\topo-}_t)=1$, then the node $b^{-}_t$ in $\BelTree^{\topo}$ has the original full observation space, and if $\beta^{\topo}(h^{\topo-}_t)=0$, the belief node will make observations with a simplified observation model $\prob{o|x}$ in a simplified observation space $\Ospace$.  
We now define a history propagation process from $h_t^{\topo-}$ to the posterior history $h_t^{\topo}$ at $t\geq1$ as:
\begin{equation}
	\zchild(h^{\tau-}_t)=\left \{ 
	\begin{array}{ll}
		\{h^{\topo}_t:  h^{\tau}_t = (h^{\topo-}_t, z_t) \ \ \ \forall z_t \in \mathcal{Z} \}, & \text{if }  \beta^{\topo}(h^{\topo-}_t)=1, \\
		\{h^{\topo}_t:  h^{\tau}_t = (h^{\topo-}_t,o_t) \ \ \ \forall o_t \in \mathcal{O} \}, & \text{if } \simpfunc^{\topo}(h^{\topo-}_t)=0. 
	\end{array}
	\right .
\end{equation}
With such a history propagating function and a given topology $\topo$, we can generate the set of all the possible posterior history  $\mathcal{H}^{\topo}_t$ and propagated history $\mathcal{H}^{\topo-}_t$ from $t=1$ to the end of the planning horizon $t=L$:
\begin{align}
	\mathcal{H}^{\topo}_{t} &= \Big\{  h^{\topo}_t: h^{\topo}_t \in \zchild(h^{\tau-}_t), \forall h^{\tau-}_t\in \mathcal{H}^{\tau-}_{t}\Big\}
	\\
	\mathcal{H}^{\tau-}_{t} &= \Big\{  h^{\tau-}_t: h^{\tau-}_t=(h^{\tau-}_{t-1}, a_{t-1}), \forall a_{t-1}\in \mathcal{A},  \forall h^{\tau}_{t-1} \in \mathcal{H}^{\tau}_{t-1}\Big\}	
	%\\ \obsNodeNot^{\topo_{}}_{t}&=\Big\{ h^{\tau-}_t: \beta^{\tau}(h^{\tau-}_t)=1, h^{\tau-}_t \in  \BelTree^{\tau-}_{t}\Big\} 
	%\\ 	\openloopNode^{\topo}_{t}&=\Big\{ h^{\tau-}_t: \beta^{\tau}(h^{\tau-}_t)=0, h^{\tau-}_t \in \BelTree^{\tau-}_{t}\Big\} 
\end{align}
and $\mathcal{H}^{\tau}_0=\{b_0\}$.

With all the possible history, 
we can represent all the belief nodes in the AOT-Tree of the topology $\topo$ by the general definition of belief: $b^{\topo}_t = \prob{x_t| h^{\topo}_t}$. So in the rest of this paper, we will interchangeably use the belief nodes and their corresponding history.

The original full POMDP belief tree can be viewed as an example where no belief node has a simplified observation model and space. The original topology is denoted as $\topo_C$, and the belief tree is denoted as $\BelTree^{\topo_C}$.
If all the belief nodes have a simplified observation model and space, we denote the topology as $\topo_S$ and its belief tree as $\BelTree^{\topo_S}$.

% An adaptive observation simplification function $\simpfunc: \CBS\to\ZspaceS$ is defined to assign a simplified observation space $\ZspaceS$ to each belief node:
% \begin{equation}
	%    \ZspaceS_{\tbm_{t-1}} = \simpfunc(\tbm_{t-1}) = \left \{ 
	% 	\begin{array}{lr}
		% 		\Zspace, & \text{if } \shis^{\topo}(\tbm_t) \in \obsNode, \\
		% 		\emptyset, & \text{if } \shis^{\topo}(\tbm_t) \notin \obsNode. 
		% 	\end{array}
	% 	\right .
	% \end{equation}
% Here, the $\obsNode$ means the set of history, after which the belief node will expand observations at time $t$. 
% If the history of a belief node $\shis_t(\tbm)$ falls in the set $\obsNodeNot_t$, the observation space at this node will be the full space $\Zspace$. 

% \DK{Included a new definition of topology-dependent observation model and the observations from this model $z^{\topo}_t$:}
With the definition of the AOT-Tree, we can define a general simplified observation model $\probo{}$, which could be different at each observation node. So, we would like to introduce the prior of propagated history $h^-_t$ and topology $\topo$ into the observation model as: $\probo{o_t|x_t, h^{-}_t, \topo}$. 
If we denote the general observation as $\gobs$, we can define an adaptive observation model that is dependent on the topology $\topo$ and the propagated history $h^{\topo-}_t$ as:
\begin{align}
	P(\gobs_t|x_t, h^{\topo-}_t, \topo) &= \simpfunc^{\topo}(h^{\topo-}_t)\probz{\gobs_t|x_t} + \big(1-\simpfunc^{\topo}(h^{\topo-}_t)\big) \probo{\gobs_t|x_t, h^{\topo-}_t, \topo}
	\label{equ:adaptive-obs-model}
	\intertext{Here, }
	\gobs_{t} \in \gobSpace_t(h^{\topo-}_t, \topo) &= \left \{ 
	\begin{array}{lr}
		\Ospace_t, & \text{if } \simpfunc^{\topo}(h^{\topo-}_t)=0, \\
		\Zspace_t, & \text{if } \simpfunc^{\topo}(h^{\topo-}_t)=1. 
	\end{array}
	\right .
	\label{equ:adaptive-obs-space}
\end{align}
A pair of indicator functions will choose whether this belief node has a simplified observation model and observation space or not. The space of the general observation $\gobs$ is alternating. 
% If we consider a specific topology $\topo$, we can denote the general observation space as $\gobSpace^{\topo}$.


We can derive the expectation below using the adaptive observation model in Equation (\ref{equ:adaptive-obs-model}) as:
\begin{align}
	&\exptsimp{\gobs_{t}|h^{\topo-}_t}{\topo} f(\gobs_t) 
	= \emathbb{x_t|h^{\topo-}_t}\exptsimp{\gobs_t|x_t, h^{\topo-}_t}{\topo} f(\gobs_t) \\ &= \emathbb{x_t|h^{\topo-}_t}\Big[\simpfunc^{\topo}(h^{\topo-}_t)\int_{\gobs_t \in \Zspace_t}\probz{\gobs_t|x_t}f(\gobs_t)d\gobs_t + \big(1-\simpfunc^{\topo}(h^{\topo-}_t)\big)\int_{\gobs_t \in \Ospace_t} \probo{\gobs_t|x_t, h^{\topo-}_t, \topo}f(\gobs_t)d\gobs_t \Big]
	\label{equ:simplifed-expt-topo}
\end{align}
Here, the function $f(\gobs_t)$ can be the reward function or value function.



For belief tree $\BelTree^\topo$, the action $\action_t$ at time $t$ is decided by a policy $\policy^{\topo}_t$ at each belief node: $\action_t = \policy_t^{\topo}(h^{\topo}_t)$. 
It depends on the history within the set $\mathcal{H}^{\topo}_t$, which is decided by the given topology $\topo$.
Policy space $\Pi$ is the set of all the possible policies that may be adopted. For a given belief tree $\BelTree^\topo$, the policy space depends on the specific topology $\topo$, denoting it as $\Pi^{\topo}=\{\pi_t: \mathcal{H}^{\topo}_t\mapsto\CA  , L\geq t \geq 0 \}$.
The planner will explore all the policies $\policy^{\topo}$ within the policy space $\Pi^{\topo}$ given the belief tree topology $\topo$ to maximize the summation of expected reward over the planning horizon to get the optimal policy $\policy^{\topo*}$. 
The optimal value function for a given topology $\topo$ can be computed by Bellman’s principle of optimality: 
% \VI{[maybe $V^{\topo*}(\tb_i)$?]}
\begin{equation}
	V^{\topo*}_{}(b^{\topo}_i) = \max_{\action_i} \Big[ r(b^{\topo}_i, \action_i) + \emathbb{x_{i+1}|b^{\topo}_i, a_i}\exptsimp{\gobs_{i+1}|x_{i+1}, (b^{\topo}_i,a_i)}{\topo} V_{}^{\topo*}(b^{\topo}_{i+1})\Big ].
\end{equation}
% Here the belief propagation function $\phi_{i+1}(\tb_i,\action_i)$ is defined as:
% \begin{align}
	%     \tb_{i+1} = \phi_{i+1}(\tb_i,\action_i) &= \bupdate_{i+1}\Big[\prob{x_i|\tb_i}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \action_i(\tb_i)}\Big] \\
	%     % &= \prob{x_i|\tb_i}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \action_i(\tb_i)}\int_{z_{i+1}\in \simpfunc(\tbm_{i+1})}\prob{z_{i+1}|x_{i+1}}
	% \end{align}

In this work, we simplify the observation space adaptively at some of the belief nodes. It will consequently simplify the policy space and thus simplify the planning. We will explore different topologies $\topo^{1},..., \topo^n $, which means different levels of simplification for the policy space, and provide simplification and the performance guarantee at the same time, meaning that our simplified planner can work out the same optimal policy as the POMDP planner. 

\subsection{Simplified Observation Model and Space as Full Observablility}
\label{subsec:full-obs-def}
In our proposed AOT-Tree introduced in the previous section, the simplification of the observation space and model is general.
Now, we would like to choose a specific group of simplifications that will be used in the rest of the paper for planning.

We define the simplified observation model $\probo{o_t|x_t, h^{\topo-}_t, \topo}$ as:
\begin{align}
    \probo{o_t|x_t, h^{\topo-}_t, \topo} = \delta(o_t-x_t)
    \ \text{ ,where }\
    o_t \in \Ospace_t = \CX_t
    \label{equ:dirac-obs-model}
\end{align}

So, the expectation in Equation (\ref{equ:simplifed-expt-topo}) will become:
\begin{align}
        &\emathbb{x_t|h^{\topo-}_t}\exptsimp{\gobs_t|x_t, h^{\topo-}_t}{\topo} f(\gobs_t) \nonumber\\& = \emathbb{x_t|h^{\topo-}_t}\Big[\simpfunc^{\topo}(h^{\topo-}_t)\int_{\gobs_t \in \Zspace_t}\probz{\gobs_t|x_t}f(\gobs_t)d\gobs_t + \big(1-\simpfunc^{\topo}(h^{\topo-}_t)\big)\int_{\gobs_t \in \Ospace_t} \probo{\gobs_t|x_t, h^{\topo-}_t, \topo}f(\gobs_t)d\gobs_t \Big] \nonumber \\
        & = \emathbb{x_t|h^{\topo-}_t}\Big[\simpfunc^{\topo}(h^{\topo-}_t)\int_{\gobs_t \in \Zspace_t}\probz{\gobs_t|x_t}f(\gobs_t)d\gobs_t + \big(1-\simpfunc^{\topo}(h^{\topo-}_t)\big)f(\gobs_t=x_t) \Big]
\end{align}

\textbf{Discussion of Complexity}

In our definition, the alternative observation space is set to be the state space by a Dirac function. For the topology $\topo$, if a single belief node $b^{\topo-}_i$ switches to the simplified observation model and space, this will reduce the dimension of the policy space $\policy_i(b^{\topo-}_i, \gobs_i)$ at this belief node from $|\mathcal{H}^{\topo-}_i||Z||A|$ to $|\mathcal{H}^{\topo-}_i||X	||A|$.
Here, the policy space at the depth of $i$ represents the number of belief nodes. 

For the original full belief tree, to calculate the expected state-dependent rewards at a depth of $i$, the expectation over the whole state space is needed, which means the complexity for expected reward is $|\mathcal{H}^{\topo-}_i||Z||A||X|$.
While for the simplified belief tree, since the full observability of state, the calculation of state-dependent reward will remain the same as $|\mathcal{H}^{\topo-}_i||X	||A|$. Compared with the original belief tree, our simplification method can save the exploration of the observation space.

This can simplify the overall planning significantly, considering the dimension of the observation space is usually high in tasks like active SLAM \cite{Placed23tro}. 

\begin{remark}[The AOT-Tree and QMDP]
Our simplification of observation space and model is connected to QMDP planning.
If the topology is chosen to be $\topo_S$ and the simplified observation model is as defined in Equation (\ref{equ:dirac-obs-model}), the AOT-Tree will become the QMDP belief tree. Hauser \cite{Hauser11icml} exploited QMDP to simplify the planning. However, our method will simplify only parts of the belief nodes adaptively and provide a theoretical guarantee.

% Similar intention has been shown in the research on macro action\cite{Flaspohler20nips, Hauser10wafr, } and durative actions\cite{Khonji23aaai}. 
\end{remark}

\subsection{Simplification as Open-Loop Planning}
\label{subsec:open-loop-def}
If we choose the simplified observation model as:
\begin{equation}
	\probo{o_t|x_t, h^{\topo-}_t, \topo} = \delta(o_t-h^{\topo-}_t)
\ \	\text{ ,where } \ \ o_t \in \mathcal{O}_t = \mathcal{H}^{\topo-}_t
\end{equation}

So, the expectation in Equation (\ref{equ:simplifed-expt-topo}) will become:
\begin{align}
	&\emathbb{x_t|h^{\topo-}_t}\exptsimp{\gobs_t|x_t, h^{\topo-}_t}{\topo} f(\gobs_t) \nonumber\\& = \emathbb{x_t|h^{\topo-}_t}\Big[\simpfunc^{\topo}(h^{\topo-}_t)\int_{\gobs_t \in \Zspace_t}\probz{\gobs_t|x_t}f(\gobs_t)d\gobs_t + \big(1-\simpfunc^{\topo}(h^{\topo-}_t)\big)\int_{\gobs_t \in \Ospace_t} \probo{\gobs_t|x_t, h^{\topo-}_t, \topo}f(\gobs_t)d\gobs_t \Big] \nonumber \\
	& = \emathbb{x_t|h^{\topo-}_t}\Big[\simpfunc^{\topo}(h^{\topo-}_t)\int_{\gobs_t \in \Zspace_t}\probz{\gobs_t|x_t}f(\gobs_t)d\gobs_t + \big(1-\simpfunc^{\topo}(h^{\topo-}_t)\big)f(\gobs_t=h^{\topo-}_t) \Big]
\end{align}
Here, the simplified observation model uses a Dirac function to make the propagated history $h^{\topo-}_t$ as the general observation for decision-making. 
If the function is reward function $r(x_{t+1})$, then:
\begin{align}
	&\emathbb{x_t|h^{\topo-}_t}\exptsimp{\gobs_t|x_t, h^{\topo-}_t}{\topo} \emathbb{x_{t+1}|x_t,\pi(h^{\topo-}_t, \gobs_t)}r(x_{t+1}) \\
	&= \emathbb{x_t|h^{\topo-}_t}\Big[\simpfunc^{\topo}(h^{\topo-}_t)\int_{\gobs_t \in \Zspace_t}\probz{\gobs_t|x_t}\emathbb{x_{t+1}|x_{t}, \pi(h^{\topo-}_t, \gobs_t)}r(x_{t+1})d\gobs_t \\ & \qquad \qquad \qquad+ \big(1-\simpfunc^{\topo}(h^{\topo-}_t)\big)\emathbb{x_{t+1}|x_{t}, \pi'(h^{\topo-}_t, \gobs_t=h^{\topo-}_t)}r(x_{t+1}) \Big]
\end{align}
Here, the policy for switching to a simplified observation model and space $\pi'(h^{\topo-}_t, \gobs_t=h^{\topo-}_t)$ becomes the mapping, $\mathcal{H}^{\topo-}_t \times 1 \mapsto \CA$.
So, for the topology $\topo$ this kind of simplification can reduce the policy space of $\policy_i(b^{\topo-}_i, \gobs_i)$ from $|\mathcal{H}^{\topo-}_t||Z||A|$ to $|\mathcal{H}^{\topo-}_i||A|$.


We will refer this to the open-loop planning, where policy will not try to reason the possible states and observations.



\begin{remark}[The AOT-Tree and Open-loop Planning]
	Flaspohler et al. \cite{Flaspohler20nips} 
\end{remark}



\section{Bounds and Performance Guarantee}
\label{sec:bound}
\subsection{Bounds for Simplification of Full Observability}
\label{subsuc:bound-full-obs}
The POMDP planner will optimize the Q-function at the top of the belief tree and decide the action at the first step. The difficulty of POMDP comes from the original Q-function being hard to calculate.
Based on our proposed AOT-tree, we can approximate the original Q-function using the Q-function of a simpler topology, which is much easier to calculate.  

However, we are interested in evaluating how good this approximation is. 
If an AOT-tree has the topology $\topo$, the Q function of executing the policy $\policy^{\topo}$ at the top of the belief tree can be written as $Q^{\policy^\topo}_{\topo}(b_0,\action_0)$. The Q-function of original full POMDP topology $\topo_C$ excuating the policy $\policy^{\topo_C}$ can be denoted as $Q^{\policy^{\topo_C}}_{\topo_C}(b_0,\action_0)$.
We would like to bound the distance $|Q^{\policy^\topo}_{\topo}(b_0,\action_0)-Q^{\policy^{\topo_C}}_{\topo_C}(b_0,\action_0)|$:
\begin{equation}
    \Delta Q(b_0,\action_0, \policy^{\topo_C},\policy^{\topo},\topo_C, \topo) :=|Q^{\policy^\topo}_{\topo}(b_0,\action_0)-Q^{\policy^{\topo_C}}_{\topo_C}(b_0,\action_0)|
\end{equation}


With this bound, we can further examine the performance guarantee for the simplification from topology $\topo$. If it cannot ensure optimal performance, the bound can serve as an indicator to guide the further exploration of different topologies until the desired performance guarantee is satisfied.

Firstly, we can bound the motion model. For  a given $h_i^{\topo_C}$ from $\BelTree^{\topo_C}$ and $h_i^{\topo}$ from $\BelTree^{\topo}$ for any topology $\topo$, considering a given motion model $\prob{x_{i+1}|x_i, a_i}$, we can bound the below total variation distance between any closed-loop policy $\pi_i^{\topo_C}$ depending on $h_i^{\topo_C}$ and a given policy $\policy^{\topo}_i$ depending on $h_i^{\topo}$:
	\begin{align}
	\big|\big|\prob{x_{i+1}|x_i, \pi_i^{\topo_C}(h_i^{\topo_C})} -& \prob{x_{i+1}|x_i, \policy^{\topo}_i(h^{\topo}_i)}\big|\big|_{TV} \nonumber\\
	&\leq \max_{\baction_i\in \CA} \big|\big|\prob{x_{i+1}|x_i, \baction_i} - \prob{x_{i+1}|x_i, \policy^{\topo}_i(h^{\topo}_i)}\big|\big|_{TV} \triangleq \delta_{M}(x_i, \policy^{\topo}_i(h^{\topo}_i))
\end{align}
%\VI{[suggest to put in context, and change to: for  a given $h_i^{\topo_C}$ from $\BelTree^{\topo_C}$ and $h_i^{\topo}$ from $\BelTree^{\topo}$ for any topology $\topo$: 
%	\begin{align}
%		\big|\big|\prob{x_{i+1}|x_i, \pi_i^{\topo_C}(h_i^{\topo_C})} -& \prob{x_{i+1}|x_i, \policy^{\topo}_i(h^{\topo}_i)}\big|\big|_{TV} \nonumber\\
%		&\leq \max_{\baction_i\in \CA} \big|\big|\prob{x_{i+1}|x_i, \baction_i} - \prob{x_{i+1}|x_i, \policy^{\topo}_i(h^{\topo}_i)}\big|\big|_{TV} \triangleq \delta_{M}(x_i, \policy^{\topo}_i(h^{\topo}_i))
%	\end{align}
%	or 
%		\begin{align}
%		\big|\big|\prob{x_{i+1}|x_i, \pi_i^{\topo_C}(h_i^{\topo_C})} -& \prob{x_{i+1}|x_i, a_i}\big|\big|_{TV} \nonumber\\
%		&\leq \max_{\baction_i\in \CA} \big|\big|\prob{x_{i+1}|x_i, \baction_i} - \prob{x_{i+1}|x_i, a_i}\big|\big|_{TV} \triangleq \delta_{M}(x_i, a_i)
%	\end{align}
%	]}
%
%    \textbf{Bound the motion model.} For a given transition model (or motion model) $P_T = \prob{x_{i+1}|x_i, a_i}$, we can bound the below total variation distance between any closed-loop policy $\pi_i^{\topo_C}$ depending on the observation $z_{i}$ and a given open-loop policy $\policy^{\topo_S}_i$:
%    \begin{align}
%        \big|\big|\prob{x_{i+1}|x_i, \pi_i^{\topo_C}} -& \prob{x_{i+1}|x_i, \policy^{\topo_S}_i}\big|\big|_{TV} \nonumber\\
%         &\leq \max_{\baction_i\in \CA} \big|\big|\prob{x_{i+1}|x_i, \baction_i} - \prob{x_{i+1}|x_i, \policy^{\topo_S}_i}\big|\big|_{TV} \triangleq \delta_{M}(x_i, \policy^{\topo_S}_i(x_i))
%    \end{align}
%    \label{lemma:motion-model}

\VI{[proof]\\}

Then, we can further derive a bound for the policy $\policy^{\topo}_i$ within a general adaptive observation topology belief tree $\BelTree^\topo$. 
\begin{lemma}
	For a given transition model $\prob{x_{i+1}|x_i, a_i}$ and a given observation model $\prob{z_i| x_i}$, we can bound the expected state-dependent reward below between the original policy $\policy^{\topo{C}}_i$ and a known policy $\policy^{\topo}_{i}$ for topology $\topo$ as: 
	%\VI{[where do you get $x_i$ from in the below? if you consider $h^-$ to be given, then should it be $\mathbb{E}^{}_{x_i \mid h^-_i}\exptsimp{\gobs_i|x_i}{}(..)$?]} %\VI{[same here; also  why does $\exptsimp{\gobs_i|x_i}{\topo}$ mean? it depends if we consider observations or not at a specific history $h^{\topo-}_i$]}
	\begin{align}
		&\big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
		&\leq \max_{\bpolicy_i} \Big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicy_i(h^-_i,\gobs^{\topo}_i)}r(x_{i+1}) - \emathbb{x_i|h^{\topo-}_i} \exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\Big| 
	\end{align}
 Here, the policy $\bpolicy_i$ is a mapping : $\mathcal{H}^-_i \times \gobSpace_i(\mathcal{H}^-_i, \topo) \mapsto \CA.$
	\label{lemma:bound-policy}
 \end{lemma}
 \begin{proof}
 First, we consider $\beta^{\topo}(h^-_i)=0$. For each $x_i \in \CX$, we can find an action $a_i$ that maximize and minimize the expected reward:
 	\begin{equation}
 		\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo_C}_i} r(x_{i+1}) dx_{i+1} \leq  \max_{a_i(x_i) \in \CA}\int_{x_{i+1}}\prob{x_{i+1}|x_i, a_i} r(x_{i+1}) dx_{i+1}
 		\label{eq-14-proof1}
 	\end{equation}
 	 	\begin{equation}
 		\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo_C}_i} r(x_{i+1}) dx_{i+1} \geq  \min_{a_i(x_i) \in \CA}\int_{x_{i+1}}\prob{x_{i+1}|x_i, a_i} r(x_{i+1}) dx_{i+1}
 		 \label{eq-15-proof1}
 	\end{equation}
 	From (\ref{eq-14-proof1}), we have:
 	\begin{align}
 		\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo_C}_i} r(x_{i+1}) dx_{i+1} &\leq  \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\max_{a_i(x_i) \in \CA}\int_{x_{i+1}}\prob{x_{i+1}|x_i, a_i} r(x_{i+1}) dx_{i+1} \\
 		& = \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\max_{a_i(x_i) \in \CA}\int_{x_{i+1}}\prob{x_{i+1}|x_i, a_i} r(x_{i+1}) dx_{i+1}
 		 		 \label{eq-17-proof1}
 	\end{align}
 	Similarly, from (\ref{eq-15-proof1}), we will get:
 	\begin{align}
 		\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo_C}_i} r(x_{i+1}) dx_{i+1} &\geq  \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\min_{a_i(x_i) \in \CA}\int_{x_{i+1}}\prob{x_{i+1}|x_i, a_i} r(x_{i+1}) dx_{i+1} \\
 		& = \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\min_{a_i(x_i) \in \CA}\int_{x_{i+1}}\prob{x_{i+1}|x_i, a_i} r(x_{i+1}) dx_{i+1}
 		 		 \label{eq-19-proof1}
 	\end{align}
 	Since we consider $\gobs^{\topo}_i=o_i$ at the belief node for the topology, the actions in Equation (\ref{eq-17-proof1}) and (\ref{eq-19-proof1}) can be viewed as a policy: $a_i(x_i)=\policy_i(h^-_i, \gobs^{\topo}_i) $. \DK{Here can also be $\policy_i(z^{\topo}_i)$? Since for all the history $h^-_i$, the inequality holds.}
 	 	 	\begin{equation}
 		\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo_C}_i} r(x_{i+1}) dx_{i+1} \leq \max_{\bpolicy_i(h^-_i, \gobs^{\topo}_i)} \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicy_i(h^-_i, \gobs^{\topo}_i)} r(x_{i+1}) dx_{i+1} 
 	\end{equation}
 	 	\begin{equation}
 		\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo_C}_i} r(x_{i+1}) dx_{i+1} \geq \min_{\bpolicy_i(h^-_i, \gobs^{\topo}_i)} \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicy_i(h^-_i, \gobs^{\topo}_i)} r(x_{i+1}) dx_{i+1} 
 	\end{equation}
 	Since different policy $\bpolicy_i(h^-_i, \gobs^{\topo}_i)$ can upper and lower bound the expected closed-loop reward, 
 	 we can also bound the distance between the the expected closed-loop reward and a known value by exploring the policy space:
 	  	 	 	\begin{align}
 	 	&\big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo_C}_i} r(x_{i+1}) dx_{i+1} - \emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1}) \big|  	 	\label{eq-22-proof1} 
 	 	\\	&\leq \max_{\bpolicy_i(h^-_i, \gobs^{\topo}_i)} \big| \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicy_i(h^-_i, \gobs^{\topo}_i)} r(x_{i+1}) dx_{i+1}- \emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})  \big|
 	 \end{align}
 	 Then, we consider $\beta(h^-_i)=1$, we have:
 	 \begin{equation}
 	  \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) = \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})
 	 \end{equation}
 	Here, $\policy^{\topo{C}}_i$ and $\policy^{\topo}_i$ share the same mapping, $\mathcal{H}^-_i\times\CZ_i\mapsto\CA$. We can say that the optimal and worst $\policy_i^{\topo}$ can upper and lower bound any $\policy^{\topo{C}}_i$. Thus, there exists a policy $\bpolicy_i^{\topo}$ that can bound the distance in Equation (\ref{eq-22-proof1}).
 	
 	Here finishes the proof of Lemma \ref{lemma:bound-policy}.
 	 \end{proof}

\begin{remark}
	\label{remark:full-obs-simp-derive}
If we take a further step from Lemma 1 and assume the propagated history $h^-_{i}$ has a pure closed-loop topology $\topo_C$:
\begin{align}
			&\max_{\bpolicy_i(h^-_i,\gobs^{\topo}_i)} \big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicy_i^{\topo}}r(x_{i+1}) - \emathbb{x_i|h^{\topo-}_i} \exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
			& \triangleq \big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicystar_i(h^-_i,\gobs^{\topo}_i)}r(x_i) - \emathbb{x_i|h^{\topo-}_i} \exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
			& = \big|\emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo_C}\emathbb{x_i|x_{i-1}, \policyc_{i-1}}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicystar_i(h^-_i,\gobs^{\topo}_i)}r(x_i) - \emathbb{x_i|h^{\topo-}_i} \exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_i)\big|
			\label{eq-26-proof2}
\end{align}
i) If both $\beta(h_{i-1}^-)=0$ and $\beta(h_{i}^-)=0$, 
 for every possible $x_i\in \CX$ and $x_{i-1} \in \CX$, we can find an action $a^{+}_{i}(x_{i})$ and $a^{+}_{i-1}(x_{i-1})$ such that:
 \begin{align}
 	&\emathbb{x_i|x_{i-1}, \policyc_{i-1}}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicystar_i}r(x_{i+1}) \nonumber \\ & \leq \max_{a_{i-1}(x_{i-1})} \emathbb{x_i|x_{i-1}, a_{i-1}(x_{i-1})}\max_{a_i(x_i)}\int_{x_{i+1}}\prob{x_{i+1}|x_i,a_i(x_i)}r(x_{i+1})
 \end{align}
 Then we have:
 \begin{align}
 	&\emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo_C}\emathbb{x_i|x_{i-1}, \policyc_{i-1}}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicystar_i(h^-_i,\gobs^{\topo}_i)}r(x_{i+1})\nonumber \\
 	& \leq \emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo_C} \max_{a_{i-1}(x_{i-1})} \emathbb{x_i|x_{i-1}, a_{i-1}(x_{i-1})}\exptsimp{\gobs_i|x_i, \{h_{i-1}, a_{i-1}\}}{\topo}\max_{a_i(x_i)}\int_{x_{i+1}}\prob{x_{i+1}|x_i,a_i(x_i)}r(x_{i+1}) \\
 	&= \emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo} \max_{a_{i-1}(x_{i-1})} \emathbb{x_i|x_{i-1}, a_{i-1}(x_{i-1})}\exptsimp{\gobs_i|x_i, \{h^-_{i-1}, z^{\topo}_{i-1}, a_{i-1}\}}{\topo}\max_{a_i(x_i)}\int_{x_{i+1}}\prob{x_{i+1}|x_i,a_i(x_i)}r(x_{i+1})
 \end{align}
 \DK{Is it possible to denote a hybrid propagated history as $h^{p-}_t$ which means the propagated history from the expectation?}
 
 Similarly, we can find the lower bound:
  \begin{align}
 	&\emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo_C}\emathbb{x_i|x_{i-1}, \policyc_{i-1}}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicystar_i(h^-_i,\gobs^{\topo}_i)}r(x_{i+1}) \\
 	& \geq \emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo_C} \min_{a_{i-1}(x_{i-1})} \emathbb{x_i|x_{i-1}, a_{i-1}(x_{i-1})}\exptsimp{\gobs_i|x_i,\{h_i, a_{i-1}\}}{\topo}\min_{a_i(x_i)}\int_{x_{i+1}}\prob{x_{i+1}|x_i,a_i(x_i)}r(x_{i+1}) \\
 	&= \emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo} \min_{a_{i-1}(x_{i-1})} \emathbb{x_i|x_{i-1}, a_{i-1}(x_{i-1})}\exptsimp{\gobs_i|x_i,\{h^-_i, z^{\topo}_{i-1}, a_{i-1}\}}{\topo}\min_{a_i(x_i)}\int_{x_{i+1}}\prob{x_{i+1}|x_i,a_i(x_i)}r(x_{i+1})
 \end{align}
 The $a_{i-1}(x_{i-1})$ and $a_i(x_i)$ in the above equations can be viewed as policy respectively, $\policy_{i-1}(h^-_{i-1},z^{\topo}_{i-1})$ and $\policy_{i}(h^-_{i-1},z^{\topo}_{i-1}, \policy_{i-1}(h^-_{i-1},z^{\topo}_{i-1}), z^{\topo}_i)$.
 Similar to Lemma \ref{lemma:bound-policy}, we can say there exists a policy to bound the below distance:
 \begin{align}
 &\big|\emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo_C}\emathbb{x_i|x_{i-1}, \policyc_{i-1}}\exptsimp{\gobs_i|x_i, h^{-}_{i} }{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicystar_i(h^{-}_i,\gobs^{\topo}_i)}r(x_{i+1}) - \emathbb{x_i|h^{\topo-}_i} \exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \nonumber\\ & \leq
 \max_{\bpolicy_{i-1}(h^-_{i-1},z^{\topo}_{i-1}), \bpolicy_{i}(h^-_{i-1},z^{\topo}_{i-1}, \bpolicy_{i-1}(h^-_{i-1},z^{\topo}_{i-1}), z^{\topo}_i)}\nonumber\\& \big|\emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo_C}\emathbb{x_i|x_{i-1}, \bpolicy_{i-1}}\exptsimp{\gobs_i|x_i,h^{p-}_{i}}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicy_i}r(x_{i+1}) - \emathbb{x_i|h^{\topo-}_i} \exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big|
 \label{eq-35-proof2}
 \end{align}
%   \begin{align}
% 	\nonumber&\big|\emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo_C}\emathbb{x_i|x_{i-1}, \policyc_{i-1}}\exptsimp{\gobs_i|x_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicystar_i(h^-_i,\gobs^{\topo}_i)}r(x_{i+1}) - \emathbb{x_i|h^{\topo-}_i} \exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\ & \geq
% 	\min_{\bpolicy_{i-1}(h^-_{i-1},z^{\topo}_{i-1}), \bpolicy_{i}(h^-_{i-1},z^{\topo}_{i-1}, \bpolicy_{i-1}(h^-_{i-1},z^{\topo}_{i-1}), z^{\topo}_i)} \nonumber\\& \big|\emathbb{x_{i-1}|h^-_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^-_{i-1}}{\topo_C}\emathbb{x_i|x_{i-1}, \bpolicy_{i-1}}\exptsimp{\gobs_i|x_i}{\topo}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicy_i}r(x_{i+1}) - \emathbb{x_i|h^{\topo-}_i} \exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big|
% 	\label{eq-36-proof2}
% \end{align}
 

 
ii) If $\beta(h_{i-1}^-)=0$ and $\beta(h_{i}^-)=1$, for each possible $x_{i-1} \in \CX$ and each $z_i \in \CZ_i$:
 \begin{align}
 	&\emathbb{x_i|x_{i-1}, \policyc_{i-1}}\exptsimp{\gobs_i|x_i}{}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicystar_i(h_{i-1}^-, z^{\topo_C}_{i-1}, \policyc_{i-1},  z^{\topo}_i)}r(x_{i+1}) \nonumber \\ & \leq \max_{a_{i-1}(x_{i-1})} \emathbb{x_i|x_{i-1}, a_{i-1}(x_{i-1})}\exptsimp{\gobs_i|x_i}{}\max_{a_i(z_i)}\int_{x_{i+1}}\prob{x_{i+1}|x_i,a_i(z_i)}r(x_{i+1})
 \end{align}
  \begin{align}
 	&\emathbb{x_i|x_{i-1}, \policyc_{i-1}}\exptsimp{\gobs_i|x_i}{}\int_{x_{i+1}}\prob{x_{i+1}|x_i, \bpolicystar_i(h_{i-1}^-, z^{\topo_C}_{i-1}, \policyc_{i-1},  z^{\topo}_i)}r(x_{i+1}) \nonumber \\ & \geq \min_{a_{i-1}(x_{i-1})} \emathbb{x_i|x_{i-1}, a_{i-1}(x_{i-1})}\exptsimp{\gobs_i|x_i}{}\min_{a_i(z_i)}\int_{x_{i+1}}\prob{x_{i+1}|x_i,a_i(z_i)}r(x_{i+1})
 \end{align}
 The $a_{i-1}(x_{i-1})$ and $a_i(z_i)$ in the above equations can be viewed as policy respectively, $\policy_{i-1}(h^-_{i-1},z^{\topo}_{i-1})$ and $\policy_{i}(h^-_{i-1},z^{\topo}_{i-1}, \policy_{i-1}(h^-_{i-1},z^{\topo}_{i-1}), z^{\topo}_i)$. Then we can get the same result as Equation (\ref{eq-35-proof2}).
    
   iii) If both $\beta(h_{i-1}^-)=1$ and $\beta(h_{i}^-)=0$, the result is similar.
  
  iv) If $\beta(h_{i-1}^-)=1$ and $\beta(h_{i}^-)=1$, the policy $\bpolicy_{i-1,i}$ in Equation (\ref{eq-35-proof2}) shares the same mapping as the closed-loop policy $\policyc_{i-1,i}$. So there exists the optimal and worst policy that upper and lower bound the expected reward, so we can also get the same result as Equation (\ref{eq-35-proof2}).
  
  \end{remark}
  If we continue the steps in Remark \ref{remark:full-obs-simp-derive} until the beginning node $b_0$, we will get:
  \begin{align}
&\Big|\exptsimp{\gobs_{1:i}|b_0, \pi^{\topo}}{\topo}(r(b^{\topo}_{i},\pi^{\topo}(h^{\topo}_i))) -  \exptsimp{\gobs_{1:i}|b_0, \pi^{\topo_C}}{\topo_C}(r(b^{\topo_C}_{i},\pi^{\topo_C}(h^{\topo_C}_i)) \Big|
   		\intertext{Assume state-dependent reward}
  =& \Big|\exptsimp{\gobs_{1:i}|b_0, \pi^{\topo}}{\topo} \emathbb{x_i|b^{\topo}_i}r(x_i) -  \exptsimp{\gobs_{1:i}|b_0, \pi^{\topo_C}}{\topo_C}\emathbb{x_i|b^{\topo_C}_i}(r(x_{i})) \Big|\\
  = & \Big|\exptsimp{\gobs_{1:i-1}|b_0, \pi^{\topo}}{\topo} \emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}r(x_i) -  \exptsimp{\gobs_{1:i-1}|b_0, \pi^{\topo_C}}{\topo_C}\emathbb{x_i|h^{\topo_C- }_i}\exptsimp{\gobs_i|x_i}{\topo_C}(r(x_{i})) \Big|
  \intertext{(Chain rule and cancel $z_i$)}
  &= \Big|\exptsimp{\gobs_{1:i-1}|b_0, \pi^{\topo}}{\topo} \emathbb{x_i|h^{\topo-}_i}r(x_i) -  \exptsimp{\gobs_{1:i-1}|b_0, \pi^{\topo_C}}{\topo_C}\emathbb{x_{i-1}|h^{\topo_C}_{i-1}}\emathbb{x_i|x_{i-1}, \policyc_{i-1}}(r(x_i)) \Big| \\  \intertext{(Bayes Rule)} 
  &=   \Big|\exptsimp{\gobs_{1:i-1}|b_0, \pi^{\topo}}{\topo} \emathbb{x_i|h^{\topo-}_i}r(x_i) -  \exptsimp{\gobs_{1:i-2}|b_0, \policy^{\topo_C}}{\topo_C}\emathbb{x_{i-1}|h^{\topo_C-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo_C-}_{i-1}}{\topo_C} \emathbb{x_i|x_{i-1},\policy^{\topo_C}_{i-1}}r(x_i) \Big|
  \label{equ:state-dependent-and-chain-rule}\\
  &=\Big|\exptsimp{\gobs_{1:i-1}|b_0, \pi^{\topo}}{\topo} \emathbb{x_i|h^{\topo-}_i}r(x_i) -\emathbb{x_0|b_0}\emathbb{x_1|x_0,\policyc_0}\exptsimp{\gobs_1|x_1, h^{p-}_{1}}{\topo_C}...\emathbb{x_{i-1}|x_{i-2},\policyc_{i-2}} \exptsimp{\gobs_{i-1}|x_{i-1},h^{p-}_{i-1}}{\topo_C}\emathbb{x_i|x_{i-1},\policy^{\topo_C}_{i-1}}r(x_i) \Big| \\
  & \leq \max_{\bpolicy^{\topo}}\Big|\exptsimp{\gobs_{1:i-1}|b_0, \pi^{\topo}}{\topo} \emathbb{x_i|h^{\topo-}_i}r(x_i) -\emathbb{x_0|b_0}\emathbb{x_1|x_0,\bpolicy^{\topo}_0}\exptsimp{\gobs_1|x_1,h^{p-}_{1}}{\topo}...\emathbb{x_{i-1}|x_{i-2},\bpolicy^{\topo}_{i-2}} \exptsimp{\gobs_{i-1}|x_{i-1},h^{p-}_{i}}{\topo}\emathbb{x_i|x_{i-1},\bpolicy^{\topo}_{i-1}}r(x_i) \Big|
    \end{align} 
  

 
\begin{lemma}
 \textbf{Bound Q value.} We can bound the Q function between the closed-loop POMDP belief tree $\topo_C$ and a given adaptive observation topology belief tree $\BelTree^\topo$ with some simplifications.
 \begin{align}
     \Delta Q(b_0,\action_0, \policy^{\topo_C},\policy^{\topo},\topo_C, \topo)
     \leq 
     \max_{\bpolicy^{\topo}\in \Pi^{\topo}} | Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) | 
     \triangleq
     \delta_Q(b_0,\action_0, \policy^{\topo},\topo)
 \end{align}
 \label{lemma:bound-q}
\end{lemma}

%The proof of Lemma \ref{lemma:bound-q} can be found at Section \ref{proof-lemma-bound-q}.

\begin{proof}
We can look into the difference in the Q function between two different topologies, which is defined as below:
 \begin{align}
		& \Delta Q(b_0,\action_0, \policy^{\topo_C},\policy^{\topo},\topo_C, \topo) \triangleq| Q_{\topo_C}^{{\policy^{\topo_C}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) | \\ 
		= & \big| \sum_{i=1}^{L} \exptsimp{\gobs_{1:i}|b_0,\policy^{\topo_C}}{\topo_C}(r({\tb}_{i})) - \sum_{i=1}^{L} \exptsimp{\gobs_{1:i}|b_0,\policy^{\topo}}{\topo}(r(b_{i})) \big| \\
    \intertext{(Assume state-dependent reward and chain rule, same as Equation (\ref{equ:state-dependent-and-chain-rule}))}
		= & \Big|\sum_{i=1}^{L}\big[\exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{i-1}|h^{\topo_C-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo_C-}_{i-1}}{\topo_C} \emathbb{x_i|x_{i-1},\policy^{\topo_C}_{i-1}}r(x_i)\ -  \exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{i-1}|h^{\topo-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo-}_{i-1}}{\topo} \emathbb{x_i|x_{i-1},\policy^{\topo}_{i-1}}r(x_i)\ \big]\Big| \\
  \intertext{(Take out the expected reward $r(x_L)$ from the summation)}
		= & \nonumber \Big|\sum_{i=1}^{L-1}\big[\exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{i-1}|h^{\topo_C-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo_C-}_{i-1}}{\topo_C} \emathbb{x_i|x_{i-1},\policy^{\topo_C}_{i-1}}r(x_i)\ -  \exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{i-1}|h^{\topo-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo-}_{i-1}}{\topo} \emathbb{x_i|x_{i-1},\policy^{\topo}_{i-1}}r(x_i)\ \big] \\ &  +  \exptsimp{\gobs_{1:L-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{L-1}|h^{\topo_C-}_{L-1}}\exptsimp{\gobs_{L-1}|x_{L-1}, h^{p-}_{L-1}}{\topo_C} \emathbb{x_L|x_{L-1},\policy^{\topo_C}_{L-1}}r(x_L)\ -  \exptsimp{\gobs_{1:L-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{L-1}|h^{\topo-}_{L-1}}\exptsimp{\gobs_{L-1}|x_{L-1}, h^{\topo-}_{L-1}}{\topo} \emathbb{x_L|x_{L-1},\policy^{\topo}_{L-1}}r(x_L)\ \Big| \\
		 \intertext{(Bound the expected reward $r(x_L)$ using Lemma \ref{lemma:bound-policy})}  
		\leq & \nonumber \max_{\bpolicy^{\topo}_{L-1}(h^{\topo_C-}_{L-1}, \gobs^{\topo}_{L-1})} \Big|\sum_{i=1}^{L-1}\big[\exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{i-1}|h^{\topo_C-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo_C-}_{i-1}}{\topo_C} \emathbb{x_i|x_{i-1},\policy^{\topo_C}_{i-1}}r(x_i)\ -  \exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{i-1}|h^{\topo-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo-}_{i-1}}{\topo} \emathbb{x_i|x_{i-1},\policy^{\topo}_{i-1}}r(x_i)\ \big] \\ &  +
		\exptsimp{\gobs_{1:L-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{L-1}|h^{\topo_C-}_{L-1}}\exptsimp{\gobs_{L-1}|x_{L-1}, h^{\topo_C-}_{L-1}}{\topo} \emathbb{x_L|x_{L-1},\bpolicy^{\topo}_{L-1}}r(x_L)\ -  \exptsimp{\gobs_{1:L-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{L-1}|h^{\topo-}_{L-1}}\exptsimp{\gobs_{L-1}|x_{L-1}, h^{\topo-}_{L-1}}{\topo} \emathbb{x_L|x_{L-1},\policy^{\topo}_{L-1}}r(x_L)\ \Big | \\
    \intertext{(Take out the expected reward $r(x_{L-1})$ from the summation, and denote the policy maximizing the distance as $\bpolicy^{+}_{L-1}(h^{\topo_C-}_{L-1}, \gobs^{\topo}_{L-1})$)} 
		=& \nonumber  \Big|\sum_{i=1}^{L-2}\big[\exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{i-1}|h^{\topo_C-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo_C-}_{i-1}}{\topo_C} \emathbb{x_i|x_{i-1},\policy^{\topo_C}_{i-1}}r(x_i)\ -  \exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{i-1}|h^{\topo-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo-}_{i-1}}{\topo} \emathbb{x_i|x_{i-1},\policy^{\topo}_{i-1}}r(x_i)\ \big] 
		\\ \nonumber & \quad + \exptsimp{\gobs_{1:L-3}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{L-2}|h^{\topo_C-}_{L-2}}\exptsimp{\gobs_{L-2}|x_{L-2}, h^{\topo_C-}_{L-2}}{\topo_C} \emathbb{x_{L-1}|x_{L-2},\policy^{\topo_C}_{L-2}}r(x_{L-1})\ -  \exptsimp{\gobs_{1:L-3}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{L-2}|h^{\topo-}_{L-2}}\emathbb{\gobs_{L-2}|h^{\topo-}_{L-2},\topo} \emathbb{x_{L-1}|x_{L-2},\policy^{\topo}_{L-2}}r(x_{L-1})
		\\ & \quad  +
		\exptsimp{\gobs_{1:L-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{L-1}|h^{\topo_C-}_{L-1}}\exptsimp{\gobs_{L-1}|x_{L-1}, h^{\topo_C-}_{L-1}}{\topo} \emathbb{x_L|x_{L-1},\bpolicy^{+}_{L-1}(h^{\topo_C-}_{L-1}, \gobs^{\topo}_{L-1})}r(x_L)\ -  \exptsimp{\gobs_{1:L-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{L-1}|h^{\topo-}_{L-1}}\exptsimp{\gobs_{L-1}|x_{L-1}, h^{\topo-}_{L-1}}{\topo} \emathbb{x_L|x_{L-1},\policy^{\topo}_{L-1}}r(x_L)\ \Big | 
		\\ = 
		\nonumber &  \Big|\sum_{i=1}^{L-2}\big[\exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{i-1}|h^{\topo_C-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo_C-}_{i-1}}{\topo_C} \emathbb{x_i|x_{i-1},\policy^{\topo_C}_{i-1}}r(x_i) -  \exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{i-1}|h^{\topo-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo-}_{i-1}}{\topo} \emathbb{x_i|x_{i-1},\policy^{\topo}_{i-1}}r(x_i) \big] 
		\\ \nonumber &  + \exptsimp{\gobs_{1:L-3}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{L-2}|h^{\topo_C-}_{L-2}}\exptsimp{\gobs_{L-2}|x_{L-2}, h^{\topo_C-}_{L-2}}{\topo_C} \emathbb{x_{L-1}|x_{L-2},\policy^{\topo_C}_{L-2}}\Big(r(x_{L-1}) +\exptsimp{\gobs_{L-1}|x_{L-1}, h^{\topo_C-}_{L-1}}{\topo} \emathbb{x_L|x_{L-1},\bpolicy^{+}_{L-1}(h^{\topo_C-}_{L-1}, \gobs^{\topo}_{L-1})}r(x_{L})\Big) 
		\\ &  \qquad \ -
		\exptsimp{\gobs_{1:L-3}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{L-2}|h^{\topo-}_{L-2}}\exptsimp{\gobs_{L-2}|x_{L-2}, h^{\topo-}_{L-2}}{\topo} \emathbb{x_{L-1}|x_{L-2},\policy^{\topo}_{L-2}}r(x_{L-1})	+  \exptsimp{\gobs_{1:L-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{L-1}|h^{\topo-}_{L-1}}\exptsimp{\gobs_{L-1}|x_{L-1}, h^{\topo-}_{L-1}}{\topo} \emathbb{x_L|x_{L-1},\policy^{\topo}_{L-1}}r(x_L)\ \Big | 			
	\intertext{(Bound the term $\emathbb{x_{L-1}|x_{L-2},\policy^{\topo_C}_{L-2}}(r(x_{L-1}) +\exptsimp{\gobs_{L-1}|x_{L-1}, h^{\topo_C-}_{L-1}}{\topo} \emathbb{x_L|x_{L-1},\bpolicy^{+}_{L-1}}r(x_{L}))$ using a similar method as Remark \ref{remark:full-obs-simp-derive})} 
		\leq
		&\nonumber\max_{\bpolicy_{L-2,L-1}} \Big|\sum_{i=1}^{L-2}\big[\exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{i-1}|h^{\topo_C-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1},h^{\topo_C-}_{i-1}}{\topo_C} \emathbb{x_i|x_{i-1},\policy^{\topo_C}_{i-1}}r(x_i) -  \exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{i-1}|h^{\topo-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo-}_{i-1}}{\topo} \emathbb{x_i|x_{i- 1},\policy^{\topo}_{i-1}}r(x_i) \big] 
		\\ &\nonumber  + \emathbb{\gobs_{1:L-3}|,b_0,\policy^{\topo_C},\topo_C}\emathbb{x_{L-2}|h^{\topo_C-}_{L-2}}\exptsimp{\gobs_{L-2}|x_{L-2}, h^{\topo_C-}_{L-2}}{\topo} \emathbb{x_{L-1}|x_{L-2},\bpolicy_{L-2}}\Big(r(x_{L-1}) +\exptsimp{\gobs_{L-1}|x_{L-1}, h^{p-}_{L-1}}{\topo} \emathbb{x_L|x_{L-1},\bpolicy_{L-1}}r(x_{L})\Big) 
		\\ & \qquad  \ -
		\exptsimp{\gobs_{1:L-3}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{L-2}|h^{\topo-}_{L-2}}\exptsimp{\gobs_{L-2}|x_{L-2}, h^{\topo-}_{L-2}}{\topo} \emathbb{x_{L-1}|x_{L-2},\policy^{\topo}_{L-2}}r(x_{L-1})	+  \exptsimp{\gobs_{1:L-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{L-1}|h^{\topo-}_{L-1}}\exptsimp{\gobs_{L-1}|x_{L-1}, h^{\topo-}_{L-1}}{\topo} \emathbb{x_L|x_{L-1},\policy^{\topo}_{L-1}}r(x_L)\ \Big | 			\\
		\intertext{(We can do it in a recursive way)} & \leq \max_{\bpolicy^{\topo}\in \Pi^{\topo}} | Q_{\topo_C}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) |
	\end{align}     

 Which completes the proof of Lemma \ref{lemma:bound-q}. 
\end{proof}




\begin{theorem}
	We can further bound the Q function of the closed-loop POMDP belief tree $\BelTree^{\topo_C}$ by deriving the tightest bound from Lemma \ref{lemma:bound-q}: 
	\begin{align}		Q_{\topo_C}^{\policy^{\topo_C}}(b_0,\action_0)  & \leq \min_{\policy^{\topo}\in \Pi^{\topo}} [Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) +\delta_Q(b_0,\action_0, \policy^{\topo},\topo) ]\\ & = \min_{\policy^{\topo}\in \Pi^{\topo}} [Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)+\max_{\bpolicy^{\topo}\in \Pi^{\topo}} | Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) |] \label{theorem-q-equ1}
	\\
	& = \max_{\policy^{\topo}\in \Pi^{\topo}}[Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)]\label{theorem-q-equ2}
	% \\		& = Q^{QMDP,*}(b_0, \pi_0)
\end{align}
\begin{align}		Q_{\topo_C}^{\policy^{\topo_C}}(b_0,\action_0)  & \geq \max_{\policy^{\topo}\in \Pi^{\topo}} [Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) -\delta_Q(b_0,\action_0, \policy^{\topo},\topo) ]\\ & = \max_{\policy^{\topo}\in \Pi^{\topo}} [Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)-\max_{\bpolicy^{\topo}\in\Pi^{\topo}} | Q_{\topo}^{{\bpolicy^{\topo}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) |] \label{theorem-q-equ3} \\
	& = \min_{\policy^{\topo}\in \Pi^{\topo}}[Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)]\label{theorem-q-equ4}
\end{align}
	\label{theorem:q}
\end{theorem}
The proof of Theorem \ref{theorem:q} can be found in Section \ref{proof:theorem-q}.


%\begin{figure}[tb]
%	\includegraphics[width=6cm]{gua.png}
%	\caption{Demonstration of Getting a Tighter Lower Bound}
%	\centering
%	\label{fig:lower-bound}
%\end{figure}

%To calculate the bound in Theorem \ref{theorem:q}, we can do it in a Bellman Optimality way. Then, we can have a tighter lower bound for the optimal closed-loop policy $\policy^{\topo_C*}$. 


Since the lower bound in Theorem \ref{theorem:q} can be loose and not informative, we can get a tighter lower bound for the optimal policy $\policy^{\topo_C*}$ for the pure closed-loop topology $\topo_C$.


\begin{lemma}
    	\textbf{Bound the optimal Q function.} 
    	For a certain topology belief tree $\topo$, if the belief node $b^{\topo-}_{i+1}$,
	The lower bound of the optimal policy within the closed-loop POMDP belief tree $\topo_C$ can be calculated in the iterative way below. We define the lower bound for the optimal Q-function for a pure closed-loop POMDP belief tree $Q_{\topo_C}^{*}(b_0,\action_0)$ as $lq(b_0, \action_0, \topo)$:
 \begin{align}
     Q_{\topo_C}^{*}(b_0,\action_0) \geq lq(b_0, u_0, \topo)
 \end{align}
 where, the lower bound function is defined iteratively as:
\begin{align}
    lq(b_t, \action_t, \topo) := &\indicator_{\simpfunc(\shis^{\topo}(b^-_{t+1}))=1}[r(b_{t},\action_t) +\exptsimp{\gobs_{t+1}|\shis^{\topo}(b_{t}),\action_t}{\topo} \max_{\policy_{t+1}}lq(b_{t+1},\policy_{t+1},\topo)]\nonumber \\
 +& \indicator_{\simpfunc(\shis^{\topo}(b^-_{t+1}))=0}[r(b_{t},\action_t) +\exptsimp{\gobs_{t+1}|\shis^{\topo}(b_{t}),\action_t}{\topo} \min_{\policy_{t}}lq(b_{t+1},\policy_{t+1},\topo)]
\label{equ:optimal-lower-bound}
\end{align} \label{lemma:bound-optimal}
\end{lemma}

The proof of Lemma \ref{lemma:bound-optimal} can be found in Section \ref{proof:lemma-optimal}.

Since the upper bound we get in Theorem \ref{theorem:q} can bound any policy, it is also the upper bound of the optimal policy, denoted as:
\begin{equation}
    uq(b_0, \action_0, \topo) \triangleq \max_{\policy^{\topo}}[Q_{\topo}^{\policy^{\topo}}(b_0,\action_0)] \geq Q_{\topo_C}^{*}(b_0,\action_0)
\end{equation}

Above all, we have obtained the bound between our proposed adaptive observation topology belief tree and the common closed-loop POMDP belief tree.


Ross et. al. \cite{Ross08jair} introduced different kinds of upper and lower bounds for online POMDP. Compared with these methods....

\subsection{Bound for Simplification of Open-Loop Planning}
For the state-dependent expected reward of $r_i$, we have:
\begin{lemma}
	If we have a known initial history $h_i^-$, for a given transition model $\prob{x_{i+1}|x_i, a_i}$ and a given observation model $\prob{z_i| x_i}$, we can bound the expected state-dependent reward below between any closed-loop policy $\policy^{\topo{C}}_i$ and a known simplified policy $\policy^{\topo}_i$ for topology $\topo$ that will simplify as Open-Loop planning by the definition from Section \ref{subsec:open-loop-def}: 
	\begin{align}
	&\big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
	&\leq R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i}\big| 
	\end{align}
	\label{lemma:bound-open-loop-reward-same-his}
\end{lemma}

\begin{proof}
	This is the proof.
	Firstly, if this step is not simplified, we have:
	\begin{align}
				&\big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
				 = &\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\big|\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1})-\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
				 = &\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\big|\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1})-\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
				 \leq & R_{\max}\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\int_{x_{i+1}}\big|\prob{x_{i+1}|x_i, \policy^{\topo{C}}_i}-\prob{x_{i+1}|x_i, \policy^{\topo}_i}\big| \\
				 \leq & R_{\max}\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\max_{a_i'(x_i)}\int_{x_{i+1}}\big|\prob{x_{i+1}|x_i, a_i'}-\prob{x_{i+1}|x_i, \policy^{\topo}_i}\big| \\
				 \leq & R_{\max}\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\max_{z_i'\in\CZ_i}\max_{a_i'(x_i)}\int_{x_{i+1}}\big|\prob{x_{i+1}|x_i, a_i'}-\prob{x_{i+1}|x_i, \policy^{\topo \prime}_i(h_i^{-}, z_i')}\big| \\
				  \leq & R_{\max}\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo}\max_{x_i'\in\CX}\max_{z_i'\in\CZ_i}\max_{a_i'(x_i)}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'}-\prob{x_{i+1}|x'_i, \policy^{\topo \prime}_i(h_i^{-}, z_i')}\big| \\
				  = & R_{\max}\max_{x_i'\in\CX}\max_{z_i'\in\CZ_i}\max_{a_i'(x_i)}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'}-\prob{x_{i+1}|x'_i, \policy^{\topo \prime}_i(h_i^{-}, z_i')}\big| \\
				  = &  R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i}\big|
	\end{align}

	Secondly, if it chooses to simplify the belief tree for open-loop planning, we have:
	\begin{align}
		&\big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
		& = \big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{x_i|h^{\topo-}_i}\emathbb{x_{i+1}|x_i, a_i}r(x_{i+1})\big| \\
		& = \big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, a_i}r(x_{i+1})\big|\\
		& \leq \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\big|\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{x_{i+1}|x_i, a_i}r(x_{i+1})\big|\\
		& = \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\big|\int_{x_{i+1}}\prob{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \int_{x_{i+1}}\prob{x_{i+1}|x_i, a_i}r(x_{i+1})\big|\\
		& \leq R_{\max} \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\int_{x_{i+1}}\big|\prob{x_{i+1}|x_i, \policy^{\topo{C}}_i} - \prob{x_{i+1}|x_i, a_i}\big| 
		\intertext{For each $x_i$, we can find an action $a_i'$ that can maximize the absolute value }
		&\leq R_{\max} \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\max_{a_i'(x_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x_i, a_i'(x_i)} - \prob{x_{i+1}|x_i, a_i}\big|\\
		\intertext{If we go on exploring all the states $x_i$, we can get a general upper bound as:}
		&\leq R_{\max} \emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\max_{x'_i\in \CX_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, a_i}\big|\\
		&= R_{\max} \max_{x'_i\in \CX_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, a_i}\big| 
		\intertext{Considering the general observation $\gobs$ identical to $h^-_{i}$, the above equation can be written in a more general way:}
		& = R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i}\big| 
	\end{align}
	
	So, in general, we can get a general bound for both situations as:
	\begin{align}
				&\big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
		&\leq R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i}\big| 
		\intertext{We can denote this as $\Delta R_{si}$ to represent the situation with the same initial history:}
		&\triangleq \Delta R_{si}(\mhis_i,\pi_i^{\topo})
	\end{align}
	This finishes the proof.
\end{proof}



Then, we take another step further to consider the situation with different initial history. 
\begin{remark}
	\label{remark:bound-open-loop-r-general}
	If we have two known initial history $h_i^-$ and $h^{\topo-}_i$, for a given transition model $\prob{x_{i+1}|x_i, a_i}$ and a given observation model $\prob{z_i| x_i}$, we can bound the expected state-dependent reward below between any closed-loop policy $\policy^{\topo{C}}_i$ and a known simplified policy $\policy^{\topo}_i$ for topology $\topo$ that will simplify as Open-Loop planning by the definition from Section \ref{subsec:open-loop-def} as: 
	%\VI{[where do you get $x_i$ from in the below? if you consider $h^-$ to be given, then should it be $\mathbb{E}^{}_{x_i \mid h^-_i}\exptsimp{\gobs_i|x_i}{}(..)$?]} %\VI{[same here; also  why does $\exptsimp{\gobs_i|x_i}{\topo}$ mean? it depends if we consider observations or not at a specific history $h^{\topo-}_i$]}
	\begin{align}
		&\big|\emathbb{h^-_i|b_0, \policyc}\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{h^{\topo-}_i|b_0,\policyt}\emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
		% =& \big|\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i(h^-_i, \gobs_i)}r(x_{i+1}) \\
		%  +& \emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i(h^-_i, \gobs_i)}r(x_{i+1}) -  \emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i(h_i^{\topo-},\gobs_i)}r(x_{i+1}) \\ +& \emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i(h_i^{\topo-},\gobs_i)}r(x_{i+1})- \emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
		\leq&\big|\emathbb{h^-_i|b_0, \policyc}\emathbb{x_i|h^-_i}\exptsimp{\gobs_i|x_i, h^-_i}{\topo_C}\emathbb{x_{i+1}|x_i, \policy^{\topo{C}}_i}r(x_{i+1}) - \emathbb{h^-_i|b_0, \policyc}\emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1}) \big|\\ &+\big| \emathbb{h^-_i|b_0, \policyc}\emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})- \emathbb{h^{\topo-}_i|b_0,\policyt}\emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
		&\leq \emathbb{h^-_i|b_0, \policyc}R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i}\big| \\ &+ \big| \emathbb{h^-_i|b_0, \policyc}\emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i(h^-_i, \gobs_i)}r(x_{i+1})- \emathbb{h^{\topo-}_i|b_0,\policyt}\emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big|\\
  		&\leq \emathbb{h^-_i|b_0, \policyc} R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i}\big| \\ &+ \max_{h^{\prime\topo-}_i}\max_{x_i'}\big| \emathbb{h^-_i|b_0, \policyc}\emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x'_i, h^{\prime\topo-}_i}{\topo}\emathbb{x'_{i+1}|x'_i, \policy^{\topo}_i(h^{\prime\topo-}_i, \gobs_i)}r(x'_{i+1})- 
  		\emathbb{h^{\topo-}_i|b_0,\policyt}\emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big|\\
&\leq \max_{h^{\prime\topo-}_i} R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i(h^{\prime\topo-}_i)}\big| \\ &+ \max_{h^{\prime\topo-}_i}\max_{x_i'}\big| \emathbb{h^-_i|b_0, \policyc}\emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x'_i, h^{\prime\topo-}_i}{\topo}\emathbb{x'_{i+1}|x'_i, \policy^{\topo}_i(h^{\prime\topo-}_i, \gobs_i)}r(x'_{i+1})- 
\emathbb{h^{\topo-}_i|b_0,\policyt}\emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
&= \max_{h^{\prime\topo-}_i} R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i(h^{\prime\topo-}_i)}\big| \\ &+ \max_{h^{\prime\topo-}_i}\max_{x_i'}\big| \exptsimp{\gobs_i|x'_i, h^{\prime\topo-}_i}{\topo}\emathbb{x'_{i+1}|x'_i, \policy^{\topo}_i(h^{\prime\topo-}_i, \gobs_i)}r(x'_{i+1})- 
\emathbb{h^{\topo-}_i|b_0,\policyt}\emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
   &\triangleq \Delta R_{di}(b_0, \policyt,\topo, i)
%		\intertext{Here, it seems exist an easy bound}
%		&\leq R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i}\big| \\ &+ \big|\int_{x_i}[\prob{x_i|h^{-}_i}\exptsimp{\gobs_i|x_i, h^{-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})- \prob{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})]\big|
%\intertext{We now make an assumption that ...., then:}
%		&\leq \emathbb{h^-_i|b_0, \policyc} R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i}\big| \\ &+ \max_{x_i'}\big| \emathbb{x_i|h^{-}_i}\exptsimp{\gobs_i|x'_i, h^{-}_i}{\topo}\emathbb{x'_{i+1}|x'_i, \policy^{\topo}_i}r(x'_{i+1})- \emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
%			&= R_{\max} \max_{x'_i\in \CX_i}\max_{\gobs_i\in\gobSpace_i}\max_{a_i'(x'_i)\in \CA_i}\int_{x_{i+1}}\big|\prob{x_{i+1}|x'_i, a_i'(x_i)} - \prob{x_{i+1}|x'_i, \policyt_i}\big| \\ &+ \max_{x_i'}\big| \exptsimp{\gobs_i|x'_i, h^{-}_i}{\topo}\emathbb{x'_{i+1}|x'_i, \policy^{\topo}_i}r(x'_{i+1})- \emathbb{x_i|h^{\topo-}_i}\exptsimp{\gobs_i|x_i, h^{\topo-}_i}{\topo}\emathbb{x_{i+1}|x_i, \policy^{\topo}_i}r(x_{i+1})\big| \\
	\end{align}	
	\label{remark:bound-open-loop-reward}
\end{remark}

Based on the previous bound, we can bound the difference of the Q-function as:

\begin{align}
    	& \Delta Q(b_0,\action_0, \policy^{\topo_C},\policy^{\topo},\topo_C, \topo) \triangleq| Q_{\topo_C}^{{\policy^{\topo_C}}}(b_0,\action_0) - Q_{\topo}^{\policy^{\topo}}(b_0,\action_0) | \\ 
		= & \big| \sum_{i=1}^{L} \exptsimp{\gobs_{1:i}|b_0,\policy^{\topo_C}}{\topo_C}(r({\tb}_{i})) - \sum_{i=1}^{L} \exptsimp{\gobs_{1:i}|b_0,\policy^{\topo}}{\topo}(r(b_{i})) \big| \\
    \intertext{(Assume state-dependent reward and chain rule)}
		= & \Big|\sum_{i=1}^{L}\big[\exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{i-1}|h^{\topo_C-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo_C-}_{i-1}}{\topo_C} \emathbb{x_i|x_{i-1},\policy^{\topo_C}_{i-1}}r(x_i)\ -  \exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{i-1}|h^{\topo-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo-}_{i-1}}{\topo} \emathbb{x_i|x_{i-1},\policy^{\topo}_{i-1}}r(x_i)\ \big]\Big| \\
		\leq & \sum_{i=1}^{L}\Big|\big[\exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo_C}}{\topo_C}\emathbb{x_{i-1}|h^{\topo_C-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo_C-}_{i-1}}{\topo_C} \emathbb{x_i|x_{i-1},\policy^{\topo_C}_{i-1}}r(x_i)\ -  \exptsimp{\gobs_{1:i-2}|b_0,\policy^{\topo}}{\topo}\emathbb{x_{i-1}|h^{\topo-}_{i-1}}\exptsimp{\gobs_{i-1}|x_{i-1}, h^{\topo-}_{i-1}}{\topo} \emathbb{x_i|x_{i-1},\policy^{\topo}_{i-1}}r(x_i)\ \big]\Big|
	\intertext{Use the Remark \ref{remark:bound-open-loop-r-general}}		
	\leq& \sum_{i=1}^{L} \Delta R_{si}(\mhis_i,\pi_i^{\topo})
\end{align}

\subsection{Idea for Planning with Limited Memory Policy}
Here, I see a chance to plan with a limited memory (window) or for a different starting belief for immediate reward

Here, to calculate the expected reward only with a limited memory (propagated belief) with a starting history $\hat{b}^-_i$. So, here, when evaluating the immediate reward at 
\begin{align}
		&\big|\emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy_i(h^-_i,z_i)}r(x_{i+1}) - \emathbb{x_i|\hat{b}^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i( z_i)}r(x_{i+1})\big| 		\\
		& = \big|\emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy_i(h^-_i,z_i)}r(x_{i+1}) - \emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i(z_i)}r(x_{i+1})
		\\& +
		 \emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i(z_i)}r(x_{i+1})-\emathbb{x_i|\hat{b}^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i( z_i)}r(x_{i+1})\big| \\
		& \leq \big|\emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy_i(h^-_i,z_i)}r(x_{i+1}) - \emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i(z_i)}r(x_{i+1}) \big|
		\\& +
		\big| \emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i(z_i)}r(x_{i+1})-\emathbb{x_i|\hat{b}^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i( z_i)}r(x_{i+1})\big| \intertext{We can use a similar trick as the open-loop planning}
		& \leq R_{\max} \emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\max_{a'_i}\int_{x_{i+1}}|p(x_{i+1}|x_i,a'_i)-p(x_{i+1}|x_i,\pi'_i(z_i))|
		\\& +
		\big| \emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i(z_i)}r(x_{i+1})-\emathbb{x_i|\hat{b}^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i( z_i)}r(x_{i+1})\big| \intertext{Then go over all the state space}
		& \leq R_{\max} \emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\max_{x'_i}\emathbb{z_i|x'_i}\max_{a'_i}\int_{x_{i+1}}|p(x_{i+1}|x'_i,a'_i)-p(x_{i+1}|x'_i,\pi'_i(z_i))|
		\\& +
		\big| \emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i(z_i)}r(x_{i+1})-\emathbb{x_i|\hat{b}^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i( z_i)}r(x_{i+1})\big| \\
		& = R_{\max} \max_{x'_i}\emathbb{z_i|x'_i}\max_{a'_i}\int_{x_{i+1}}|p(x_{i+1}|x'_i,a'_i)-p(x_{i+1}|x'_i,\pi'_i(z_i))|
		\\& +
		\big| \emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i(z_i)}r(x_{i+1})-\emathbb{x_i|\hat{b}^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i( z_i)}r(x_{i+1})\big| \\
		& \leq R_{\max} \max_{x'_i}\emathbb{z_i|x'_i}\max_{a'_i}\int_{x_{i+1}}|p(x_{i+1}|x'_i,a'_i)-p(x_{i+1}|x'_i,\pi'_i(z_i))|
		\\& +
		\max_{x'_i}\big| \emathbb{h^-_i|b_0, \policy}\emathbb{x_i|h^-_i}\emathbb{z_i|x'_i}\emathbb{x_{i+1}|x'_i, \policy'_i(z_i)}r(x_{i+1})-\emathbb{x_i|\hat{b}^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i( z_i)}r(x_{i+1})\big| \\
		& = R_{\max} \max_{x'_i}\emathbb{z_i|x'_i}\max_{a'_i}\int_{x_{i+1}}|p(x_{i+1}|x'_i,a'_i)-p(x_{i+1}|x'_i,\pi'_i(z_i))|
		\\& +
		\max_{x'_i}\big| \emathbb{z_i|x'_i}\emathbb{x_{i+1}|x'_i, \policy'_i(z_i)}r(x_{i+1})-\emathbb{x_i|\hat{b}^-_i}\emathbb{z_i|x_i}\emathbb{x_{i+1}|x_i, \policy'_i( z_i)}r(x_{i+1})\big| \intertext{We can treat the bound as a function:}
		&\triangleq B(\hat{b}^-_i, \pi',i)
\end{align}

This bound can be further written in an adaptive way. 

\subsection{Adaptive Simplification of History-dependent Policy for POMDP (or Adaptive Simplification of History for POMDP)}
We can see Open-loop planning and limited history policy as two cases of history-dependent policy. 
So the two bound together can form an Adaptive Simplification of History-dependent Policy for POMDP. 

It means:
\begin{equation}
	o_i = \varphi(h_i)
\end{equation}

For open-loop planning, this simplification function is:
\begin{equation}
	o_i = \varphi(h_i) = \{a_{1:i}\}
\end{equation}

For finite memory based policy,  this simplification function is:
\begin{equation}
   	o_i = \varphi(h_i) = \{z_{i}\}
\end{equation}
Relevant paper: \cite{Subramanian22jmlr} comes up with a notion of Approximated Information State that is a function of history. 
\cite{Patil24ais} takes this theory to MDP and derives features from history to help reinforcement learning. 

\subsection{Performance guarantee after simplification}
Here, we consider the performance guarantee at the top of the belief tree. 
The key idea is to make sure that the proposed belief tree with some simplifications in the observation space can still make the same optimal decisions as the common POMDP belief tree even after simplifications.

We use the bound of the Q function derived in Section \ref{subsuc:bound-full-obs} to analyze the performance guarantee. 
The objective of the guarantee is based on the analysis of the overlapping states of different $\action_0$.
Figure \ref{fig:guarantee} shows how the performance guarantee is used at the top of the belief tree. 

\begin{figure}[b]
	\includegraphics[width=8cm]{Figures/gua.png}
	\caption{The performance guarantee at the top of the belief tree}
	\centering
        \label{fig:guarantee}
\end{figure}

\subsection{Update and Exploration of Observation Topology}
We propose to use the overlapping of the Q function at the top of the belief tree as a measure to evaluate validity of the current belief tree $\topo$. 

Compared with the commonly used metric in open-loop policy exploration in POMDP, the Value of Information, our method saves the exploration of the observation space and does not sacrifice performance at all.






==> logs/04-Sampling.tex <==
\subsection{Sparse Sampling for the Adaptive Observation Belief Tree}
We propose an importance sampling method as the estimator of the Q value used in the previous section.

\subsubsection{Self-Normalized Importance Sampling}

\DK{Add more introduction to self-normalized sampling here...}

From a practical aspect, the actual value of the Q function is hard to get. Similarly, the bound we get from the previous section is also impractical to calculate. Monte Carlo sampling is a commonly used method that can approximate the target functions efficiently. 

For a random variable $X\sim \mathcal{P}$, we use another sampling-based random variable, $Y\sim \mathcal{Q}$ to approximate the expectation of the original theoretic value. If we obtain some samples $\{y_i\}_{i=1}^N$ from a known distribution $\mathcal{Q}$, the calculation will be: 
\begin{equation}
\emathbb{X\sim \mathcal{P}}[f(X)] = \int f(x)\mathcal{P}(x)dx = \int f(x)\frac{\mathcal{P}(x)}{\mathcal{Q}(x)}\mathcal{Q}(x)dx \simeq \frac{1}{N}\sum_{i=1}^{N}\frac{\mathcal{P}(y_i)}{\mathcal{Q}(y_i)} f(y_i)
\end{equation}

Usually, the proposed distribution $\mathcal{Q}$ is the known motion model. 
The weighted sampling can be more efficient where resampling will create more particles from the samples with higher weights. The belief density is approximated by $\Bar{b}(x)\simeq \frac{\sum_{i=1}^N w^i \delta(x-x^i)}{\sum_{i=1}^N w^i}$.
\DK{This part needs more details.}

\subsubsection{Bounded Estimation Error}
We define the estimated upper bound and lower bound as $\hat{uq}(b_0,a_0, \topo)$ and $\hat{lq}(b_0,a_0, \topo)$. 
The estimation of the upper bound can be seen as an estimation of the optimal Q function within the given belief tree $\BelTree^\topo$:
\begin{flalign}
	\hat{uq}(b_0,a_0, \topo) &= 
	\max_{\policy^{\topo}_{1:L-1}}	[\hat{Q}_{\topo}^{\policy^{\topo}_{1:L-1}}(b_0,\action_0)] 
	\\ &=  \hat{Q}_{\topo}^{\policy^{\topo}*}(b_0,\action_0)
\end{flalign}

We can define the estimation error for it as:
\begin{flalign}
	\Delta \hat{uq}(b_0,a_0, \topo) &\triangleq|\hat{uq}(b_0,a_0, \topo) - {uq}(b_0,a_0, \topo)| 
	\\ & = |\hat{Q}_{\topo}^{\policy^{\topo*}}(b_0,\action_0) - {Q}_{\topo}^{\policy^{\topo*}}(b_0,\action_0) |
\end{flalign}

But the estimation of the lower bound $\hat{lq}(b_0,a_0, \topo)$ should be calculated iteratively by Equation (\ref{equ:optimal-lower-bound}). The estimation error is defined as:
\begin{flalign}
	\Delta \hat{lq}(b_0,a_0, \topo) &\triangleq|\hat{lq}(b_0,a_0, \topo) - {lq}(b_0,a_0, \topo)| 
\end{flalign}



\begin{theorem}
	[\textbf{Bounded Estimation Error}] For all the depth $d=0,...,L-1$ and $a$, the following concentration bound holds with probability at least $1-|A|(|A|C)^L\exp(\frac{-C\lambda^2}{2V_{\max}^2})$ :
	\begin{flalign}
		\Delta \hat{uq}(b_0,a_0, \topo) \leq \frac{L(L-1)}{2}\lambda
	\end{flalign}
	\label{theorem:upper-bound-estimation}
\end{theorem}
It can provide a guarantee for our theory when it is practically implemented.
The proof of Theorem \ref{theorem:upper-bound-estimation} can be found in Section \ref{proof: upper-bound-estimation}.

For the lower bound, we use a similar way to show the estimation bound.

\begin{theorem}
	[\textbf{Estimation bound of the lower bound}] For all the depth $d= 0,..., L-1$ and $\action$, the following concentration bound holds with probability at least $1-|A|(|A|C)^L\exp(\frac{-C\lambda^2}{2V_{\max}^2})$:
	\begin{equation}
		\Delta \hat{lq}(b_0,a_0, \topo) \leq \frac{L(L-1)}{2}\lambda
	\end{equation}
	\label{theorem:lower-bound-estimation}
\end{theorem}
Proof can be found in Section \ref{proof: lower-bound-estimation}. 



% \begin{lemma}
	%     \textbf{Particle Likelihood SN Estimator Convergence Bound} (Adapted from Lemma 1 of \cite{Lim23jair}).  
	% Suppose a function $f$ is bounded by a finite constant 
	% $\|f\|_{\infty} \leq f_{\max}$, 
	% and a particle belief state 
	% $\Bar{b}_d = \{s_{d,i}, w_{d,i}\}$
	% at the depth $d$ represents $b_d$ with particle likelihood weighting that is recursively updated as 
	% $w_{d,i}= \indicator_{\simpfunc^{\topo}(h^-(s_d))=1}w_{d-1,i}\cdot P_z(o_d|a, s_d)+\indicator_{\simpfunc^{\topo}(h^-(s_d))=0} w_{d-1,i}$.
	% Then, for all $d = 0,..., D-1$, the following weighted average is the SN estimator of f under the belief $b_d$ corresponding to the actions $\{a_n\}_{n=0}^{d-1}$ and observations $\{o_n\}^d_{n=1}$, for all beliefs $b_d\in B$ that are
	% realizable given the initial belief $b_0$:
	% \begin{equation}
		%     \Tilde{\mu}_{\Bar{b}_d}(f) = \frac{\sum_{i=1}^{C}w_{d,i}f(s_{d,i})}{\sum_{i=1}^{C}w_{d,i}}
		% \end{equation}
	% and the following concentration bound holds with probability at least $1-3\exp(-C\cdot t^2_{\max}(\lambda,C))$:
	% \begin{equation}
		%     |\emathbb{s\sim b_d}(f(s))-\Tilde{\mu}_{\Bar{b}_d}(f)| \leq \lambda,
		% \end{equation}
	% \begin{equation}
		%     t_{\max}(\lambda,C) := \frac{\lambda}{f_{\max}d_{\infty}^{\max}}-\frac{1}{\sqrt{C}}
		% \end{equation}
	% \end{lemma}

